Flame Front Propagation and Finger Competition and Formation of a Single Saffman-Taylor Finger without Surface Tension - PhD Thesis

Problems of interface growth have received much attention recently Such are, for example, the duffusion limited aggregation (DLA), random sequential adsorption (RSA), Laplacian growth or flame front propagation. We will mainly pay attention in this Thesis to the numerical and analytical investigation of the last two problems. In addition to the fact that flame front propagation is an interesting physical problem we feel that we can also explain experimental results on the basis of theoretical investigations. There exists possibility to use methods found for the flame front propagation, in different fields where similar problems appear such as the important model of Laplacian growth .

==> SS.tex <==


\chapter{Summary}
The problem of flame propagation is studied as an example of unstable fronts
that
wrinkle on many scales. The analytic tool of pole expansion
in the complex plane is employed to address the interaction of the unstable
growth
process with random initial conditions and
perturbations. We argue that the effect of random noise is immense and that it
can never be neglected in sufficiently large systems. We present simulations
that lead to scaling laws
for the velocity and acceleration of the front as a function of the system
size and the level of noise, and analytic arguments that explain these results
in terms of the noisy pole dynamics.

We consider flame front propagation in channel geometries. The steady state
solution in this problem is space dependent, and therefore the linear
stability analysis is
described by a partial integro-differential equation with a space dependent
coefficient. Accordingly it involves complicated eigenfunctions. We show
that the analysis
can be performed to required detail using a finite order dynamical
system in
terms of the dynamics of singularities in the complex plane, yielding
detailed understanding
of the physics of the eigenfunctions and eigenvalues.

The roughening of expanding flame fronts by the accretion of cusp-like
singularities
is a fascinating example of the interplay between instability, noise and
nonlinear
dynamics that is reminiscent of self-fractalization in Laplacian growth
patterns.
The nonlinear integro-differential equation
that describes the dynamics of expanding flame fronts is amenable to analytic
investigations using pole decomposition. This powerful technique
allows the development of a satisfactory understanding of the qualitative and
some quantitative aspects of the complex geometry that develops in
expanding flame fronts.

Flame Propagation is used as a prototypical example of expanding fronts
that wrinkle without limit in radial geometries but reach a simple
 shape in channel geometry. We show
 that the relevant scaling laws that govern the radial growth can be
 inferred once the
 simpler channel geometry is understood in detail. In radial geometries (in
 contrast to
 channel geometries) the effect of external
 noise is crucial in accelerating and wrinkling the fronts. Nevertheless,
 once the interrelations between
 system size, velocity of propagation and noise level are understood in channel
 geometry, the scaling laws for radial growth follow.

 The mathematical problem of Laplacian growth without surface tension exhibits
 a family of exact (analytic) solutions in terms of logarithmic poles in the
 complex plane. We show that this family of solutions has a remarkable property:
 generic initial conditions in channel geometry which begin with arbitrarily
 many features exhibit an inverse cascade into a single finger.


==> ftsl.tex <==


%\documentstyle[12pt,twoside]{article}
\pagestyle {empty}
%\begin{document}
%\renewcommand{\baselinestretch}{1}
\centerline{\large\bf Thesis leading to}
\vspace{0.2cm}
\centerline{\large\bf the degree of Ph.D.}
\vspace{2.5cm}
\centerline{\Large\bf  Interface Growth Processes }
\vspace{2.0cm}
\centerline{Oleg Kupervasser }
\vspace{0.7cm}
\centerline{\bf Under The Supervision of: Itamar Procaccia}
\vspace{0.4cm}
\centerline{\em Department of Chemical Physics}
\centerline{\em The Weizmann Institute of Science }
\centerline{\em 76100 Rehovot, Israel}\par
\vspace{2.0cm}
$$    $$
$$    $$
$$    $$
$$    $$
\centerline{\em November 1999}\par
\vspace{0.8cm}
%\renewcommand{\baselinestretch}{1.9}
\newpage
%\end{document}


==> int.tex <==


%\documentstyle[aps,pre,preprint,floats]{revtex}
%\begin{document}
  \chapter{Introduction}
 Problems of interface growth have received
 much attention recently \cite{Pel,BS,Vic}.
 Such are, for example, the duffusion limited aggregation (DLA) \cite{WIS},
 random sequential adsorption (RSA) \cite{JWE},
 Laplacian growth \cite{94DMW,DM94,M98} or
 flame front propagation \cite{77Siv}.
 We will mainly pay attention in this Thesis to the
 numerical and analytical investigation of the last two problems.
 In addition to the fact that flame front propagation
 is an interesting physical problem
 we feel that we can also explain experimental results on the
 basis of  theoretical
  investigations.
 There exists possibility to use methods found for the flame front propagation,
 in different fields where similar problems appear such as the important
 model of Laplacian growth .

 The premixed flame - the self-sustaining wave of an exothermic chemical
 reaction - is one of the basic manifestations of gaseous combustion.
 It is well established, however, that the simplest imaginable flame
 configuration - unbounded planar flame freely propagating through
 initially motionless homogeneous combustible mixture - is intrinsically
 unstable and spontaneously assumes a characteristic two- or three-dimensional
 structure.

 In the recent paper of Gostintsev, Istratov and Shulenin \cite{89GIS} an interesting
 survey of experimental studies on outward propagating spherical and cylindrical
 flames in the regime of well developed hydrodynamic (Darrieus-Landau)
 instability is presented. The available data clearly indicate that freely
 expanding wrinkled flames possess two intrinsic features:

 \begin{enumerate}
 \item Multi-quasi-cusps structure of the flame front. (The flame front
 consists of a large number of quasi-cusps, i.e., cusps with rounded
 tips.)
 \item Noticeable acceleration of the flame front
 \end{enumerate}

 Moreover, the temporal dependence of the flame radius is nearly identical
 for all premixtures discussed and correlates well with the simple
 relation:

\begin{equation}
     R_0 (t)=At^{3/2}+B \label{int1e}
\end{equation}

 Here $R_0 (t)$ is the effective (average) radius of the wrinkled
 flame and A, B are empirical constants.

 In this Thesis we study the spatial and temporal behavior of
 a nonlinear continuum model (i.e.,
 a model which possesses an infinite
 number of degrees of freedom) which embodies all the characteristics deemed
 essential to premixed flame systems; namely,
  dispersiveness, nonlinearity and linear
 instability.
 Sivashinsky, Filyand and Frankel \cite{94FSF} recently obtained
 an equation, denoted by SFF in what follows, to describe how
 two-dimensional wrinkles of the cylindrical premixed flame grow
 as a consequence of the well-known Landau-Darrieus hydrodynamic
 instability. The SFF equation reads as follows:

 \begin{equation}
  {\partial R \over \partial t}=
    {U_b\over 2{R_0}^2(t)}\left({\partial R \over \partial \theta }\right)^2
       +{D_M\over {R_0}^2(t)}{\partial^2 R\over \partial\theta^2}+{\gamma
       U_b\over 2R_0 (t)} I\{R\}+U_b{ } \ . \label{erf3e}
\end{equation}
where 0$ <\theta <  2\pi$ is an angle, R($\theta$,t) is the modulus of
 the radius-vector
on the flame interface, $U_b,D_M,\gamma$ are constants.
\begin{eqnarray}
    && I(R)={1\over \pi}\sum_{n=1}^\infty n\int_{0}^{2\pi} cos[n(\theta-
         \theta^*)]R(\theta^*,t)d\theta^*= \nonumber\\ &&
   =-{1\over\pi}P\int_{-\infty}^{+\infty}
    {{\partial R(\theta^*,t)\over \partial\theta^*}\over \theta^*-\theta}
  d\theta^*  \label{erf4e}
\end{eqnarray}

\begin{equation}
  R_0 (t)={1\over 2\pi}\int_{0}^{2\pi}R(\theta,t)d\theta \ . \label{erf5e}
  \end{equation}




 Sivashinsky, Filyand and Frankel \cite{94FSF} made a direct numerical
 simulation of this nonlinear evolution equation for the cylindrical
 flame interface
 dynamics. The result obtained shows that the two mentioned experimental
 effects take place. Moreover, the evaluated acceleration rate is not
 incompatible with the power law given by eq.(\ref{int1e}).
  For comparison, numerical simulations of freely expanding diffusively
 unstable flames were presented as well.
  In this case no tendency towards acceleration has been
 observed.

 In the absence of surface tension, whose effect is to stabilize the
 short-wavelength perturbations of the interface, the problem of 2D
 Laplacian growth is described as follows

 \begin{equation}
 (\partial^2_x+\partial^2_y)u=0 \ . \label{ozz2e}
 \end{equation}

 \begin{equation}
 u \mid_{\Gamma(t)}=0 \ , \partial_nu \mid_{\Sigma}=1 \ . \label{ozz3e}
 \end{equation}

 \begin{equation}
 v_n= \partial_nu \mid_{\Gamma(t)}  \ . \label{ozz4e}
 \end{equation}

 Here $u(x,y ;t)$ is the scalar field mentioned, $\Gamma(t)$ is the
 moving interface, $\Sigma$ is a fixed external boundary, $\partial_n$ is a
 component of the gradient normal to the boundary
(i.e. the normal derivative), and $v_n$ is a normal component of the velocity of
  the front.


 To obtain results for radial flame growth it is necessary to
 investigate the channel case first. The channel version of equation
 for flame front propagation is the so-called Michelson-Sivashinsky
 equation \cite{85TFH,90GS} and looks like
 \begin{equation}
       {\partial H \over \partial t}=
    {1 \over 2}\left({\partial H\over \partial x }\right)^2
    +\nu { \partial^2 H\over \partial x^2}+ I\{H\}\ . \label{erf1e}
 \end{equation}
\begin{equation}
    I(H)=
      -{1\over\pi}P\int_{-\infty}^{+\infty}
   {{\partial H(x^*,t)\over \partial x^*}\over x^*-x}
       dx^*\ . \label{erf2e}
\end{equation}

 with periodic boundary condition on the interval x [0,L],
      where L is size of the system. $\nu$ is constant, $\nu>0$.
           H is the height of the flame front point,
            $P\int$ is the usual principal value integral.



 Equations for flame front propagation and Laplacian growth with zero surface
 tension have remarkable property : these equations can be solved in
 terms of poles in the complex plane \cite{94DMW,85TFH,84BF,89J,95J}. So we obtain  a set of
 ordinary differential equations for the coordinates of these poles.
 The number of the poles is constant value in the system, but to explain
 such effect as growth of the velocity flame front we need to consider
 some noise that is a source of new poles. So we need to solve the problem
 of interaction of the  random fluctuations and the pole motion.

 The simplest case is the channel geometry. Main results for this case
 is existence of the giant cusp solution \cite{85TFH}(Fig.1.1), which is represented in configuration space by poles which are organized on a line parallel to the imaginary
 axis. This pole solution is an attractor for pole dynamics.
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %\narrowtext
 \begin{figure}
 \epsfxsize=9.0truecm
 \epsfbox{fag.ps}
 \caption
 {Giant cusp solution}
 \label{file=Fig.2e}
 \end{figure}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 A complete analysis of this steady-state solution was first presented in
 Ref.\cite{85TFH} and the main
 results are summarized as follows:
 \begin{enumerate}
 \item There is only one
 stable stationary solution which is geometrically represented by a giant
 cusp (or equivalently one finger) and
 analytically by $N(L)$ poles which are aligned on one line parallel to the
 imaginary
 axis. The existence of this solution is made clearer with the following
 remarks.
 \item There exists an attraction between the poles along the real line.
  The resulting dynamics merges all the $x$
 positions of poles whose $y$-position remains finite. \item The $y$
 positions are distinct, and the poles are aligned above each other in
 positions
 $y_{j-1}<y_j<y_{j+1}$ with the maximal being $y_{N(L)}$. This can be
 understood from
 equations for the poles motion in which the interaction is seen to be repulsive at short ranges,
 but changes sign at longer ranges.
 \item If one adds
 an additional pole to such
 a solution, this pole (or another) will be pushed to infinity along the
 imaginary axis.
 If the system has less than $N(L)$ poles it is unstable to the addition of
 poles,
 and any noise will drive the system towards this unique state. The number
 $N(L)$ is
 \begin{equation}
 N(L)= \Big[{1 \over 2}\left( {L \over \nu }+1\right) \Big]\ , \label{NofLe}
 \end{equation}
 where $\Big[ \dots \Big]$ is the integer part  and $2\pi L$ is a system size. To see this consider a
 system with $N$ poles and such
 that all the values of $y_j$ satisfy the condition $0< y_j <y_{max}$. Add
 now one
 additional pole whose coordinates are $z_a\equiv (x_a,y_a)$ with $y_a\gg
 y_{max}$. From the equation of motion for $y_a$,  we see that the
 terms in
 the sum are all of the order of unity as is also the $\cot(y_a)$ term. Thus
 the equation of motion of $y_a$ is approximately
 \begin{equation}
 {dy_a \over dt}\approx \nu{2N+1 \over L^2}-{1\over L} \ . \label{yae}
 \end{equation}
 The fate of this pole depends on the number of other poles. If $N$ is too
 large the pole
 will run to infinity, whereas if $N$ is small the pole
 will be attracted towards the real axis. The condition for moving away to
 infinity
 is that $N > N(L)$ where $N(L)$ is given by (\ref{NofLe}). On the other hand
 the $y$
 coordinate of the poles cannot hit zero. Zero is a repulsive line, and poles
 are pushed away from zero with infinite velocity.
 To see this consider
 a pole whose $y_j$ approaches zero. For any finite $L$ the term
 $\coth(y_j)$ grows
 unboundedly whereas all the other terms in the equation for the poles motion remain bounded.
 \item The height of the cusp is proportional to $L$. The distribution of
 positions
 of the poles along the line of constant $x$ was worked out in \cite{85TFH}.
 \end{enumerate}
 We will refer to the solution with all these properties as the
 Thual-Frisch-Henon
 (TFH)-cusp solution.

 The main results of our own work are as follow.
 Traditional linear analysis was made for this giant cusp solution.
 This analysis demonstrates the existence of negative eigenvalues
 that go to zero when the system size goes to infinity.

 \begin{enumerate}
 \item There exists an obvious Goldstone or translational mode
 with eigenvalue $\lambda_0=0$.
 This eigenmode stems from the Galilean invariance of the equation of motion.
 \item The rescaled eigenvalues ($L^2\lambda_i$) oscillate periodically between
 values that are
 $L$-independent in this
 presentation. In other words, up to the
 oscillatory
 behavior the eigenvalues depend on $L$ like $L^{-2}$.
 \item The eigenvalues $\lambda_1$ and $\lambda_2$
  hit zero periodically. The functional
  dependence in this presentation appears almost piecewise linear.
  \item  The higher eigenvalues also exhibit similar qualitative behavior,
  but without
  reaching zero.
  We note that the solution becomes marginally stable for every value of $L$ for
  which the eigenvalues
  $\lambda_1$ and $\lambda_2$ hit zero. The $L^{-2}$ dependence of the spectrum
  indicates that the solution becomes more and more sensitive to noise as $L$
  increases.
  \end{enumerate}

 It was proved that arbitrary initial conditions can be written
 in the term of poles in the complex plane.
 Inverse cascade process of giant cusp formation was investigated
 numerically and analytically. Dependencies of the flame front width
 and mean velocity were found. The next step in investigation of
 the channel case was the influence of random noise on the pole dynamics.
 The main effect of the external noise is the appearance of new poles in the
 minima of the flame front and the  merging these poles with the giant cusp.
 The dependence of the mean flame front velocity on the noise and the system
 size was found. The velocity is almost independent on the noise
 until the noise  achieves
 some critical value. In the dependence of the velocity
 on the system size we see growth of the velocity with some exponent
 until the velocity achieves some saturation value.

 Denoting  $v$ as the  velocity of the flame front and  L  the system
  size:

 \begin{enumerate}
 \item
 We can see two different regimes of  behavior the average velocity
 $v$ as a function of noise
 $f$ for fixed system size L. For the noise $f$ smaller then same fixed value
 $f_{cr}$
 \begin{equation}
 v\sim f^\xi \ . \label{rre}
 \end{equation}
 For these values of $f$ this dependence is very weak, and
 $\xi\approx 0.02$.
  For
    large values of $f$ the dependence is much stronger
      \item
       We can see growth of the average velocity $v$ as a function of
     the system size L. After some values of L we can see saturation of the
       velocity.
         For regime $f<f_{cr}$ the growth of the velocity can be written as
           \begin{equation}
         v\sim L^\mu , \quad \mu\approx 0.35\pm 0.03 \ . \label{zcalere}
           \end{equation}
             \end{enumerate}

 The dependence of the number of poles in the system and the number of the poles
 that appear in the system in unit  time was investigated numerically
 as a function of the noise and the system parameters.
 The life time of a  pole was found numerically.
 Theoretical
 discussion of the effect of noise on the pole dynamics and mean
 velocity was made \cite{OGKP}.

 Pole dynamics can be used also to analyze small perturbation of
 the flame front and make the full
 stability analysis of the giant cusp. Two kinds of
 modes were found. The first one is eigenoscillations of the poles in the giant
 cusp. The second one is modes connected to the  appearance of the new poles
 in the system.
 The eigenvalues of these modes were found.
 The results are in good agreement wit
 h the
 traditional stability analysis \cite{KOP99}.

 The results found for the cannel case can be used to analyze
 flame front propagation in the radial case \cite{KOP95,KOP951}. Main feature of
 this case is a competition between attraction of the poles and
 expanding of the flame front. So in this case we obtain not
 only one giant cusp but a set of cusps. New poles that appear
 in the system because of the noise form these cusps. On the
 basis of the equation of poles motion we can find connection between
 acceleration of the flame front and the width of the interface.
 On the basis of the result for mean velocity in the channel case
 the acceleration of the flame front can be found. So we obtain
 full picture of the flame front propagation in the radial case.

 The next step in the  investigation of the problem  is considering
  Laplacian growth with zero surface tension that also has
 pole solutions. In the case of Laplacian growth we obtain result
 that is analogous to the merging of the poles in the channel
 case of the flame front propagation: all poles coalesce into one
 pole in the case of periodic boundary condition or two poles
 on the boundaries in the case of no-flux boundary conditions.
 This result can be proved theoretically \cite{KOP953}.

 In papers \cite{Seva1,Seva2,Seva3,Seva4,Seva5}
 self-acceleration without involvement of the external
 forcing is considered.
 No self-acceleration exist for the finite number of poles. So we can explain
 the self-acceleration and the appearance of new poles or by the noise or
 by the "rain" of poles from the "cloud" in infinity.
 Indeed, any given initial condition can be written as a
 sum of infinite number of poles( Sec. 2.4.1).
 Let us consider one pole that appears from the "cloud" in infinity.
 We neglect by the repulse force from the rest of poles in the system
 and consider only attraction force in Eqs.\ref{eqsze} $-{\gamma \over 2r_0}$
 For $r_0$ we can write in the case of self-acceleration
 $r_0(\tau)=(a+\tau)^{\beta},r_0(0)=a^{\beta},\beta>1$.
 So from $\tau=0$ to $\tau=\infty$ pole comes down a distance $\Delta y=
 \int_0^{\infty}{\gamma \over 2r_0(\tau)}d\tau={\gamma \over 2} {1 \over
 \beta-1} {1 \over r_0(0)^{\beta-1 \over \beta}}$.
 So the "rain" come down the finite distance after the infinite time and this
 distance converges to zero if $r_0(0) \mapsto \infty$!
 So we think that the appearance of new poles from the infinity
 can be explained only by the external noise.
 The characteristic size of cusp in the system ${\cal L} \sim
 r_0^{{1\over \beta}}$. So from Fig 2.23 the noise $f \sim {1 \over {\cal L}^5}
 \sim {1 \over r_0^{5\over \beta}}$ is necessary for the appearance of new cusps
 in the system. If the noise is larger than this value the
 dependence on the noise is
 very slow( $f^0.2$ for regime II and $f^0.02$ for regime III). This result
 explains the weak dependence of numerical simulations on the noise reduction
 (\cite{Seva1}, Fig.2).

Joulin et al. \cite{jula1,jula2,jula3,jula4}
use a vary similar approach for the channel and radial
flame growth. But the main attention in our work is made to the velocity of
flame front (self-acceleration for the radial case) and the flame front width.
Main attention in the channel case in Joulin's work was made to the
investigation of mean-spacing between cusps (crests).
For the radial case only the linear dependence of radius on time
(no self-acceleration) is
considered in Joulin's work.
Our works greatly complement each other but don't compete with
each other.For example, for the distance between cusps
(the mean value of cusp) without any proof we use Eq.(2.70).
Fig.9(\cite{jula2})
give us a excellent proof of this equation.


 The structure of this Thesis is as follow.
 Chapter 1 is this Introduction.

 In Chapter 2 we obtain main results for the channel case of
 the flame front propagation. We give results about steady state
 solutions, present traditional linear analysis of the problem and
 investigate analytically and numerically the influence of noise
 on the mean velocity of the front and pole dynamics.

 In Chapter 3 we obtain results of the linear stability analysis
 by the help of pole solutions.

 In Chapter 4 we use the result obtained for the channel case
 for analysis of the flame front propagation in the radial
 case

 In Chapter 5 we investigate asymptotic behavior of the
 poles in the complex plane for the Laplacian growth with
 the zero surface-tension in the case of periodic
 and no-flux boundary condition.

 Chapter 6 is a summary.


%\end{document}


==> ole1.tex <==


%\documentstyle[aps,prl,twocolumn,floats,psfig,epsf]{revtex}
%\begin{document}
%\draft
\chapter{ Pole-Dynamics in Unstable Front Propagation: the Case of the
Channel Geometry}
\section{Introduction}
The aim of this chapter is to examine the role of random fluctuations on the
dynamics
of growing wrinkled interfaces which are governed by non-linear equations
of motion.
We are interested in those examples for which the growth of a flat or smooth
interface are inherently unstable. A famous example of such growth phenomena is
provided by Laplacian growth patterns \cite{Pel,BS,Vic}. The experimental
realization of such
patterns is seen for example in Hele-Shaw cells \cite {Pel} in which air or
another low viscosity
fluid is displacing oil or some other high viscosity fluid.
Under normal conditions the advancing fronts do not remain flat; in channel
geometries
they form in time a stable finger whose width is determined by delicate effects
that arise from the existence of surface tension. In radial geometry, the
growth the interface
forms a contorted and ramified fractal shape. A related phenomenon has been
studied
in a model equation for flame propagation which has the same linear stability
properties as the Laplacian growth problem \cite{77Siv}. The physical
problem in this case
is that of pre-mixed flames which
exist as self-sustaining fronts of exothermic chemical reactions in gaseous
combustion. Experiments \cite{89GIS} on flame propagation in radial
geometry show that the flame
front accelerates as time
goes on, and roughens with characteristic exponents. Both observations did not
receive proper theoretical explanations. It is notable that  the channel and
radial
growth are markedly different; the former leads to a single giant
cusp in the
moving front, whereas the latter exhibits infinitely many cusps that appear in
a complex hierarchy as the flame front develops (\cite{94FSF,KOP95} and
chapter 4).

Analytic techniques to study such processes are available \cite{82LC}. In
the context of
flame propagation \cite{KOP95,85TFH,89J,90J}, and in Laplacian growth in
the zero surface-tension limit \cite{84SB,86How,94DMW} one
can examine solutions that are described in terms of poles in the complex plane.
This description is very useful in providing a set of ordinary differential equations
for the positions of the poles, from which one can deduce the geometry of the
developing front in an extremely economical and efficient way.
Unfortunately this
description is not available in the case of Laplacian growth with surface
tension, and this makes the flame propagation problem very attractive.
However, it  suffers from one fundamental drawback. For the noiseless
equation the pole-dynamics always conserves the number of poles that existed in the initial
conditions.  As a result there is a final degree of ramification that is afforded
by every set of initial conditions even in the radial geometry, and it is not
obvious
how to describe the continuing self-similar growth that is seen in
experimental conditions or numerical simulations. Furthermore, as mentioned before,
at least in the
case of flame propagation one observes \cite{89GIS} an {\em acceleration}
of the flame
front with time. Such a phenomenon is impossible when the number
of poles is conserved. It is therefore tempting to conjecture that noise
may have
an important role in affecting the actual growth phenomena that are observed in
such systems. In fact, the effect of noise on unstable front dynamics has not
been adequately addressed in the literature. From the point of view of analytic
techniques noise can certainly generate new poles even if the initial conditions
had a finite number of poles. The subject of pole dynamics with the existence
of random noise, and the interaction between
random fluctuations
and deterministic front propagation are the main issues of this chapter.

We opt to study the example of flame propagation rather than Laplacian growth, simply because
the former has an analytic description in terms of poles also in the experimentally
relevant
case of finite viscosity. We choose to begin the study with channel
geometry. The reason is that in radial geometry it is more difficult to
disentangle
the effects of external noise from those of initial conditions. After all,
initially the system can contain
 infinitely many poles,very far away near infinity in the complex
plane (and therefore having an infinitely small contribution to the interface).
Since the growth of the radius changes the stability of the system,
more and more of these poles might  fall down to the real axis and become observable.
In channel geometry the analysis of the effect of
initial conditions
is relatively straightforward, and one can understand it before focusing on
the (more interesting) effects of external noise \cite{85TFH}.  The basic reason
for this is that
in this geometry the noiseless steady state solution for the developed front
is known analytically. As described in Section II, in a channel of width $L$
the steady-state solution is given in terms of
$N(L)$ poles that are organized on a line parallel to the imaginary axis.
It  can
be shown that for any number of poles in the initial conditions this is the only
attractor of the pole dynamics. After the establishment of this
steady state we can begin to systematically examine the effects of external
noise on this solution. As stated before, in
radial conditions there is no stable steady state with a finite number of poles,
and the disentanglement of initial vs. external perturbations is less
straightforward (\cite{KOP95} and chapter 4).
We show later that the insights provided in this chapter have relevance
for radial growth as well as will be discussed in the sequel.

We have a number of goals in this chapter. Firstly, after introducing the pole
decomposition, the pole dynamics, and the basic steady state, we will
present stability
analysis of the solutions of the flame propagation problem in a channel
geometry. It will
be shown that the giant cusp solution is linearly stable, but non-linearly
unstable. These results, which are described in Section III, can be obtained
either by
linearizing the dynamics around the giant cusp solutions in order to study the stability
eigenvalues, or by examining perturbations in the form of poles in the
complex plane. The
main result of Section III is that there exists one Goldstone mode and two
modes whose
eigenvalues hit the real axis periodically when the system size $L$
increases. Thus
the system is marginally stable at particular values of $L$, and it is always
nonlinearly unstable, allowing finite size perturbations to introduce new
poles into the system. This insight allows us to understand the relation
between the
system size and the effects of noise. In Section IV we discuss the
relaxation dynamics
that ensues after starting the system with ``small" initial data.  We
study the
coarsening process that leads in time to the final solution of the giant cusp, and
understand from this what are the typical time scales that exist in our
dynamics.
We offer in this Section some results of numerical simulations that are
interpreted
in the later sections.
In Section V we focus on the phenomenon of acceleration of the flame front
and its relation
to the existence of noise. In noiseless conditions the velocity of the flame
front in a finite channel is bounded \cite{85TFH}. This can be shown either by using the pole
dynamics or directly from the equation of motion. We will present the results
of numerical simulations where the noise is controlled, and show how the
velocity of the flame front is affected by the level of the noise and the
system size.
The main results are: (i) Noise is responsible for introducing new poles to the
system; (ii) For low levels of noise the velocity of the flame front scales
with the
system size with a characteristic exponent; (iii) There is a phase transition at
a sharp (but system-size dependent) value of the noise-level, after which the behavior
of the system changes qualitatively; (iv) After the phase transition the
velocity
of the flame front changes very rapidly with the noise level. In the last
Section we remark on the implications of these observations for the scaling behavior
of the radial growth problem, and  present a summary and conclusions.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Equations of Motion and Pole-decomposition in the Channel Geometry}
It is known that planar flames freely propagating
through initially motionless homogeneous combustible mixtures are
intrinsically unstable.
It was reported that such flames develop characteristic structures which
include cusps,
and that under usual experimental conditions the flame front accelerates as
time goes
on. A model in $1+1$ dimensions that pertains to the propagation of flame
fronts in channels of width
$\tilde L$ was proposed in \cite{77Siv}. It is written in terms of position
$h(x,t)$ of the
flame front above the $x$-axis. After appropriate rescalings it takes
the form:
\begin{equation}
{\partial h(x,t) \over \partial t}=
{1\over 2}\left[{\partial h(x,t) \over \partial x }\right]^2
 +\nu{\partial^2 h(x,t)\over \partial x^2}+ I\{h(x,t)\}+1 \ . \label{Eqnondime}
\end{equation}
The domain is  $0 <x< \tilde L$, $\nu$ is a parameter and we use periodic boundary
conditions. The functional $I[h(x,t)]$
is the Hilbert transform which is conveniently defined in terms of the spatial
Fourier transform
\begin{eqnarray}
&&h(x,t)= \int_{-\infty}^{\infty} e^{i k x}\hat h(k,t) dk \label{Foure}\\
&& I[h(k,t)] = |k| \hat h(k,t) \label{hile}
\end{eqnarray}
For the purpose of introducing the pole-decomposition it is convenient to
rescale the domain to $0<\theta <2\pi$. Performing this rescaling and
denoting the
resulting quantities with the same notation we have
\begin{eqnarray}
&&{\partial h(\theta,t) \over \partial t}=
{1\over 2L^2}\left[{\partial h(\theta,t) \over \partial \theta }\right]^2
 +{\nu\over L^2}{\partial^2 h(\theta,t)\over \partial\theta^2}\nonumber \\&&+
{1\over L}I\{h(\theta,t)\}+1 \ . \label{Eqdime}
\end{eqnarray}
In this equation $L=\tilde L/2\pi$.
Next we change variables to $u(\theta,t)\equiv {\partial
h(\theta,t)/\partial\theta}$.
 We find
\begin{equation}
{\partial u(\theta,t) \over \partial t}=
{u(\theta,t)\over L^2}{\partial u(\theta,t) \over \partial \theta }
 +{\nu\over L^2}{\partial^2 u(\theta,t)\over \partial \theta^2}+ {1\over
L}I\{u(\theta,t)\} \ . \label{eqfinale}
\end{equation}
It is well known that the flat front solution of this equation is linearly
unstable.
The linear spectrum in $k$-representation is
\begin{equation}
\omega_k=|k|/L-\nu k^2/L^2 \ . \label{spece}
\end{equation}
There exists a
typical scale $k_{max}$ which is the last unstable mode
\begin{equation}
k_{max} = {L\over \nu} \ . \label{kmaxe}
\end{equation}
Nonlinear effects stabilize a new steady-state which is discussed next.

The outstanding feature of the solutions of this equation is the appearance
of cusp-like structures in the developing fronts. Therefore a representation in
terms of Fourier modes is very inefficient. Rather, it appears very
worthwhile to represent such solutions in terms of sums of functions of poles
in the complex plane. It will be shown below that the position of the cusp along the
front is determined by the real coordinate of the pole, whereas the height of the
cusp is in correspondence with the imaginary coordinate. Moreover, it will
be seen that the dynamics of the developing front can be usefully described in
terms of the dynamics of the poles. Following \cite{82LC,85TFH,90J,KOP95} we
expand the solutions $u(\theta,t)$ in functions that depend on
$N$ poles whose position $z_j(t)\equiv x_j(t)+iy_j(t)$ in the complex plane
is time dependent:
\begin{eqnarray}
&&u(\theta,t)=\nu\sum_{j=1}^{N}\cot \left[{\theta-z_j(t) \over 2}\right]
   + c.c.\nonumber \\
&&=\nu\sum_{j=1}^{N}{2\sin [\theta-x_j(t)]\over \cosh
[y_j(t)]-\cos [\theta-x_j(t)]}\ , \label{upolese}
\end{eqnarray}
\begin{equation}
h(\theta,t)=2\nu\sum_{j=1}^{N}{\ln \Big[\cosh (y_j(t))-\cos
(\theta-x_j(t)) \Big]}+C(t) \ . \label{rpolese}
\end{equation}
In (\ref{rpolese}) $C(t)$ is a function of time. The function
(\ref{rpolese}) is a superposition of quasi-cusps (i.e. cusps that
are rounded at the tip). The real part of the pole position (i.e.
$x_j$) is the coordinate (in the domain $[0,2\pi]$) of the maximum
of the quasi-cusp, and the imaginary part of the pole position
(i.e $y_j$) is related to the depth of the quasi-cusp. As $y_j$
decreases the depth of the cusp increases. As $y_j \to 0$ the
depth diverges to infinity. Conversely, when $y_j\to \infty$ the
depth decreases to zero.

The main advantage of this representation is that the propagation
and wrinkling of the front can be described via the dynamics of
the poles. Substituting (\ref{upolese}) in (\ref{eqfinale}) we
derive the following ordinary differential equations for the
positions of the poles:
\begin{equation}
- L^2{dz_{j}\over dt}=\Big[\nu\sum_{k=1
  ,k\neq j}^{2N }\cot \left({z_j-z_k\over 2}\right)
  +i{L\over 2 }sign [Im(z_j)]\Big].\label{eqze}
\end{equation}
We note that in (\ref{upolese}), due to the complex conjugation,
we have $2N$ poles which are arranged in pairs such that for $j<N$
$z_{j+N}=\bar z_j$. In the second sum in (\ref{upolese}) each pair
of poles contributed one term. In Eq.(\ref{eqze}) we again employ
$2N$ poles since all of them interact. We can write the pole
dynamics in  terms of the real and imaginary parts $x_j$ and
$y_j$. Because of the arrangement in pairs it is sufficient to
write the equation for either $y_j>0$ or for $y_j<0$. We opt for
the first. The equations for the positions of the poles read
\begin{eqnarray}
&&-L^2{dx_{j}\over dt}=\nu\sum_{k=1,k\neq j}^N
   \sin(x_j-x_k)\Bigg[
   [\cosh (y_j-y_k) \label{xje} \\ && -\cos (x_j-x_k)]^{-1}+[\cosh
(y_j+y_k)-\cos (x_j-x_k)]^{-1}\Bigg]  \nonumber\\
&& L^2{dy_{j}\over dt}=\nu\sum_{k=1,k\neq j}^{N }\Big({\sinh (y_j-y_k)\over
   \cosh (y_j-y_k)-\cos (x_j-x_k)}\nonumber \\ &&+
   {\sinh (y_j+y_k)\over \cosh (y_j+y_k)-\cos (x_j-x_k)}
   \Big)+\nu\coth (y_j)- L\label{yje}  .
\end{eqnarray}
We note that if the initial conditions of the differential
equation (\ref{eqfinale}) are expandable in a finite number of
poles, these equations of motion preserve this number as a
function of time. On the other hand, this may be an unstable
situation for the partial differential equation, and noise can
change the number of poles. This issue will be examined at length
in Section \ref{noisee}.
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Linear Stability Analysis in Channel Geometry}

In this section we discuss the linear stability of the TFH-cusp
solution. To this aim we first use  Eq.(\ref{upolese}) to write
the steady solution $u_s(\theta)$ in the form:
\begin{equation}
u_s(\theta)=\nu\sum_{j=1}^{N}{2\sin [\theta-x_s]\over \cosh
[y_j]-\cos [\theta-x_s]}\ , \label{state}
\end{equation}
where $x_s$ is the real (common) position of the stationary poles and $y_j$
their
stationary imaginary position. To study the stability of this solution we need
to determine the actual positions $y_j$. This is done numerically by integrating the
equations of motion for the poles starting from $N$ poles in initial
positions and
waiting for relaxation. Next one perturbs this solution with a
small perturbation $\phi(\theta,t)$: $u(\theta,t) =
u_s(\theta)+\phi(\theta,t)$ .
 Linearizing the dynamics for small $\phi$ results in the equation of motion
\begin{eqnarray}
 &&{\partial \phi(\theta,t) \over \partial t}= {1\over L^2}\Big
[\partial_\theta [u_s(\theta) \phi(\theta,t)]
 +\nu \partial_\theta^2\phi(\theta,t)\Big]\nonumber \\
 && +{1\over L}I(\phi(\theta,t)) \ . \label{lineare}
\end {eqnarray}
\subsection{Fourier decomposition and eigenvalues}
The linear equation can be decomposed in Fourier modes according to
\begin{eqnarray}
\phi(\theta,t)&=&\sum_{k=-\infty}^{\infty} \hat\phi_k(t) e^{ik\theta}\\
u_s(\theta)&=&-2{\nu}i\sum_{k=-\infty}^{\infty}
  \sum_{j=1}^N {\rm sign}(k)e^{-\mid k \mid y_j}e^{ik\theta}
\end {eqnarray}
In these sums the discrete $k$ values run over all the integers.
Substituting in (\ref{lineare}) we get the equations:
\begin{equation}
{d\hat \phi_k(t) ) \over dt}= \sum _n a_{kn} \hat\phi_n(t)\ , \
\end {equation}
 where  $a_{kn}$ is a infinite matrix whose entries are given by
\begin{eqnarray}
a_{kk}&=&{\mid k \mid\over L} -{\nu \over L^2} k^2\\
a_{kn}&=&{k\over L^2}{\rm sign}(k-n)({2\nu} \sum_{j=1}^N e^{-\mid k-n \mid y_j})
 \quad k \neq n \ .
\end {eqnarray}
To solve for the eigenvalues of this matrix we need to truncate it
at some cutoff $k$-vector $k^*$. The choice of $k^*$ can be based
on the linear stability analysis of the flat front. The scale
$k_{max}$, cf. (\ref{kmaxe}), is the largest $k$ which is still
linearly unstable. We must choose $k^*>k_{max}$ and test the
choice by the converegence of the eigenvalues. The chosen value of
$k^*$ in our numerics was $4k_{max}$. The results for the low
order eigenvalues of the matrix $a_{kn}$ that were obtained from a
converged numerical calculation are presented in Fig.2.1.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
%\epsfxsize=9.0truecm
%\epsfbox{Fir7.ps}
\psfig{file=fig1.ps,width=7.0cm,angle=-90} \caption {The first 10
highest eigenvalues of the stability matrix with $\nu=\pi/5$,
multiplied by the square of the system size $L^2$ vs. the system
size $L$. Note that all the eigennvalues oscillate around fixed
values in this presentation, and that the highest two eigenvalues
hit zero periodically. } \label{file=Fig.1e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The eigenvalues are multiplied by $L^2$ and are plotted
as a function of $L$. We order the eigenvalues
in decreasing order and denote them as $\mid \lambda_0 \mid \le
\mid \lambda_1 \mid \le \mid \lambda_2 \mid
\dots$.

Fig 2.1 contains a strange result on the positive eigenvalues at large L.
One of methods to check some numerical result is to do analytic investigation.
For example, in Chapter 3 we make detailed analytic investigation for
the numerical result on Fig. 2.1 and obtain that all eigenvalues are not
positive. Indeed, two types of modes exists. The first one is connected to
the displacement of poles in the giant cusp. Because of the pole attraction
the giant cusp is stable with respect to the longitudinal displacement of
poles and so the correspondent eigenvalues are not positive. For the transversal
displacement the Lyapunov function exists and so the giant cusp is stable with
respect to the transversal displacement and the correspondent eigenvalues are
not positive. The second type of modes is connected to additional poles.
These poles go to infinity because of the repulsion from the giant cusp poles
$N(L)$. So the correspondent eigenvalues are also not positive.
So the positive eigenvalues at large L are a numerical artifact.

The figure offers a number of qualitative observations:
\begin{enumerate}
\item There exists an obvious Goldstone or translational mode $u_s'(\theta)$
with eigenvalue $\lambda_0=0$, which is shown with rhombes in Fig.2.1.
This eigenmode stems from the Galilean invariance of the equation of motion.
\item The eigenvalues oscillate periodically between values that are
$L$-independent in this
presentation (in which we multiply by $L^2$). In other words, up to the
oscillatory
behavior the eigenvalues depend on $L$ like $L^{-2}$.
\item The eigenvalues $\lambda_1$ and $\lambda_2$, which are represented by squares
and circles in Fig.2.1, hit zero periodically. The functional
dependence in this presentation appears almost piecewise linear.
\item The higher eigenvalues also exhibit similar qualitative behaviour,
but without
reaching zero.
We note that the solution becomes marginally stable for every value of $L$ for
which the eigenvalues
$\lambda_1$ and $\lambda_2$ hit zero. The $L^{-2}$ dependence of the spectrum
indicates that the solution becomes more and more sensitive to noise as $L$
increases.
\end{enumerate}
\subsection{Qualitative understanding using pole-analysis}

The most interesting qualitative aspects are those enumerated
above as item 2 and 3. To understand them it is useful to return
to the pole description, and to focus on Eq.(\ref{yae}). This
equation describes the dynamics of a single far-away pole. We
remarked before that this equation shows that for {\em fixed} $L$
the stable number of poles is the integer part (\ref{NofLe}).
Define now the number $\alpha$, $0\le\alpha\le 1$, according to
\begin{equation}
\alpha= \Big[{1 \over 2}\left( {L \over \nu }+1\right) \Big]-
{1 \over 2}\left( {L \over \nu }-1\right)
 \ . \label{alphae}
\end{equation}
Using this number we rewrite Eq.(\ref{yae}) as
\begin{equation}
{dy_a\over dt} \approx {2\nu \over L^2}\alpha \ . \label{yalphae}
\end{equation}
As $L$ increases, $\alpha$ oscillates piecewise linearly and periodically
between zero and unity. This shows that a distant pole which is added to
the giant
cusp solution is usually repelled to infinity except when $\alpha$ hits
zero and the system becomes marginally unstable to the addition of a new pole.

To connect this to the linear stability analysis we note from
Eq.(\ref{upolese}) that a single far-away pole solution (i.e with
$y$ very large) can be written as
\begin{equation}
u(\theta,t) = 4 \nu e^{-y(t)} \sin(\theta-x(t)) \ . \label{farye}
\end{equation}
Suppose that we add to our giant cusp solution a perturbation of
this functional form. From Eq.(\ref{yalphae}) we know that $y$
grows linearly in time, and therefore this solution decays
exponentially in time. The rate of decay is a linear eigenvalue of
the stability problem, and from Eq.(\ref{yalphae}) we understand
both the $1/L^2$ dependence and the periodic marginality. We
should note that this way of thinking gives us a significant part
of the $L$ dependence of the eigenvalues, but not all. The
variable $\alpha$ is rising from zero to unity periodically, but
after reaching unity it hits zero instantly. Accordingly, if the
highest non zero eigenvalue were fully determined by the pole
analysis, we would expect this eigenvalue to behave as the solid
line shown in Fig.2.2.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
%\epsfxsize=9.0truecm
%\epsfbox{Fir7.ps}
\psfig{file=fss.ps,width=7.0cm,angle=-90} \caption { Comparison of
the numerically determined highest 4 eigenvalues of the stability
matrix with the prediction of the pole analysis. The eigenvalues
of the stability matrix are :$\lambda_0$, $\lambda_1$, $\lambda_2$
 and
 $\lambda_3$. The pole analysis (solid line) provides a
 qualitative understanding of the stability, and appears to overlap with the high
 est
 eigenvector over half of the range, and with the fourth eigenvalue
 over the other half.}
\label{file=Fig.1e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The actual highest eigenvalue computed from the stability matrix
is shown in rhombuses connected by dotted line. It is clear that
the pole analysis gives us a great deal of qualitative and
quantitative understanding, but not all the features agree.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Dynamics near marginality}

The discovery of marginality at isolated values of $L$ poses
questions regarding the fate of poles that are added at very large
$y$'s at certain $x$-positions. We will argue now that when the
system becomes marginally stable, a new pole can be added to those
existing in the giant cusp. We remember that these poles have a
common $\theta$ position that we denote as $\theta=\theta_c$. The
fate of a new pole added at infinity depends on its $\theta$
position. If the position of the new pole is again denoted as
$y_a$, and $\infty \gg y_a \gg y_{max}$, we can see from
Eq.(\ref{yje}) that $dy_a/dt$ is maximal when $\theta_a=\theta_c$,
whereas it is minimal when $\theta_a-\theta_c =\pi$. This follows
from the fact that the cosine term has a value $+1$ when
$\theta_a=\theta_c$ and a value $-1$ when
 $\theta_a-\theta_c =\pi$. For large $y$ differences
the terms in the sum take on their minimal value when the $\cos$
term is $-1$ and their maximal values at $+1$. For infinitely
large $y_a$ the equation of motion is (\ref{yae}) which is
independent of $\theta_a$. Since the RHS of this equation becomes
zero at marginality, we conclude that for very large but finite
$y_a$ $dy_a/dt$ changes sign from positive to negative when
$\theta_a-\theta_c$ changes from zero to $\pi$. The meaning of
this observation is that the most unstable points in the system
are those points which are furthest away from the giant cusp. It
is interesting to discuss the fate of a pole that is added to the
system at such a position. From the point of view of the pole
dynamics $\theta=\theta_c+\pi$ is an unstable fixed point for the
motion along the  $\theta$ axis. The attraction to the giant cusp
exactly vanishes at this point. If we start with a pole at a very
large $y_a$ close to this value of $\theta$ the down-fall along
the $y$ coordinate will be faster than the lateral motion towards
the giant cusp. We expect to see therefore the creation of a small
cusp at $\theta$ values close to $\pi$ that precedes a later stage
of motion in which the small cusp moves to merge with the giant
cusp. Upon the approach of the new pole to the giant cusp all the
existing poles will move up and the furthest pole at $y_{max}$
will be kicked off to infinity. We will later explain that this
type of dynamics occurs in stable systems that are driven by
noise. The noise generates far away poles (in the imaginary
direction) that get attracted around $\theta=\theta_c+\pi$ to
create small cusps that run continuously towards the giant cusp.
%%%%%%%%%%%%%%%%%%%%%
\subsection{Excitable System.}

The intuition gained so far can be used to discuss the issue of stability of a
stable system to {\em larger} perturbations. In other words, we may want to
add to the
system poles at finite values of $y$ and ask about their fate. We first
show in this
subsection that poles whose initial $y$ value is below $y_{max}\sim \log
(L^2/\nu^2)$
will be attracted towards the real axis. The scenario is
similar to
the one described in the last paragraph.

Suppose that we generate a stable system with a giant cusp at
$\theta_c=0$ with poles distributed along the $y$ axis up to
$y_{max}$. We know that the sum of all the forces that act on the
upper  pole is zero. Consider then an additional pole inserted in
the position $(\pi,y_{max})$. It is obvious from Eq.(\ref{yje})
that the forces acting on this pole will pull it downward. On the
other hand if its initial position is much above $y_{max}$ the
force on it will be repulsive towards infinity. We see that this
simple argument identifies $y_{max}$ as the typical scale for
nonlinear instability.

Next we estimate $y_{max}$ and interpret our result in terms of
the {\em amplitude} of a perturbation of the flame front. We
explained that uppermost pole's position fluctuates between a
minimal value and infinity as $L$ is changing. We want to estimate
the characteristic scale of the minimal value of $y_{max}(L)$. To
this aim we employ the result of ref.\cite{85TFH} regarding the
stable distribution of pole positions in a stable large system.
The parametrization of \cite{85TFH} differs from ours; to go from
our parametrization in Eq.(\ref{eqfinale}) to theirs we need to
rescale $u$ by $L^{-1}$ and $t$ by $L$. The parameter $\nu$ in
their parameterizations is $\nu/L$ in ours. According to
\cite{85TFH} the number of poles between $y$ and $y+dy$ is given
by the $\rho(y)dy$ where the density $\rho(y)$ is
\begin{equation}
\rho(y)={L\over \pi^2\nu}\ln[\coth(|y|/4)] \ . \label{diste}
\end{equation}
To estimate the minimal value of $y_{max}$ we require that the tail of the
distribution $\rho(y)$ integrated between this value and infinity will allow
one single pole. In other words,
\begin{equation}
\int_{y_{max}}^\infty dy \rho(y) \approx 1 \ . \label{intege}
\end{equation}
Expanding (\ref{diste}) for large $y$ and integrating explicitly
the result in (\ref{intege}) we end up with the estimate
\begin{equation}
y_{max} \approx 2\ln\Big[{4L\over \pi^2\nu}\Big]
\end{equation}
For large $L$ this result is $y_{max}\approx \ln({L^2 \over
\nu^2})$. If we now add an additional pole in the position
$(\theta,y_{max})$ this is equivalent to perturbing the solution
$u(\theta,t)$ with a function $\nu e^{-y_{max}} \sin(\theta)$, as
can be seen directly from (\ref{upolese}). We thus conclude that
the system is unstable to a perturbation {\em larger} than
\begin{equation}
u(\theta) \sim \nu^3 \sin(\theta)/L^2 \ . \label{nu3L2e}
\end{equation}
This indicates a very strong size dependence of the sensitivity of the giant
cusp solution to external perturbations. This will be an important ingredient in our
discussion of noisy systems.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Initial Conditions, Pole Decomposition and Coarsening}

In this section we show first that any initial conditions can be
approximated by pole decomposition. Later, we show that the
dynamics of sufficiently smooth initial data can be well
understood from the pole decomposition. Finally we employ this
picture to describe the {\it inverse cascade} of cusps into the
giant cusp which is the final steady state.  By inverse cascade we
mean a nonlinear coarsening process in which the small scales
coalesce in favor of larger scales and finally the system
saturates at the largest available scale\cite {coars}.
%%%%%%%%%%%%%%%%%%%%
\subsection{Pole Expansion: General Comments}
The fundamental question is how many poles are needed to
describe any given initial condition. The answer, of course, depends on how
smooth are
the initial conditions. Suppose also that we have an initial function
$u(\theta,t=0)$ that is $2\pi$-periodic and which at time $t=0$ admits a Fourier
representation
\begin{equation}
u(\theta) = \sum_{k=1}^{\infty} A_k \sin{(k\theta+\phi_k)} \ ,
\label{Fouriere}
\end{equation}
with $A_k > 0$ for all $k$. Suppose that  we want to find a
pole-decomposition representation $u_p(\theta)$ such that
\begin{equation}
|u_p(\theta) - u(\theta)| \le \epsilon  \qquad {\rm
for~~every~~}\theta \ , \label{epse}
\end{equation}
where $\epsilon$ is a given wanted accuracy.  If $u(\theta)$ is
differentiable we can
cut the Fourier expansion at some finite $k=K$ knowing that the remainder
is smaller
than, say, $\epsilon/2$.  Choose now a large number $M$ and a small number
$\Delta\ll 1/M$
and write the pole representation for $u_p(\theta)$ as
\begin{equation}
u_p(\theta) = \sum_{k=1}^K \sum_{p=0}^{M-1} {2k
\sin{(k\theta+\phi_k})\over \cosh{[k(y_k
+p\Delta)]}-cos{(k\theta+\phi_k})} \ . \label{upe}
\end{equation}
To see that this representation is a particular form of the
general formula (\ref{upolese}) We use the following two
identities
\begin{equation}
\sum_{k=0}^{\infty} e^{-kt} \sin{xk} = {1\over 2} {\sin{x}\over
\cosh{t}-\cos{x}} \ , \label{identAe}
\end{equation}
\begin{equation}
\sum_{k=0}^{K-1}\sin (x+ky)=\sin (x+{K-1 \over 2}y)\sin{Ky \over 2}
     {\rm cosec}{y \over 2}\ . \label{identBe}
\end{equation}
From these follows a third identity
\begin{eqnarray}
&&\sum_{j=0}^{K-1}{2\sin{(x-{2\pi j\over K}+\phi)}\over\cosh{y}-\cos{(x-{2\pi
j\over K}+\phi)}}\nonumber \\
&&= {2K\sin{(Kx+\phi)}\over \cosh{Ky}-\cos{(Kx+\phi)}} \ .
\label{identCe}
\end{eqnarray}
Note that the LHS of (\ref{identCe}) is of the form
(\ref{upolese}) with $K$ poles whose positions are all on the line
$y_j=y$ and whose $x_j$ are on the lattice points $2\pi j/K-\phi$.
On the other hand every term in (\ref{upe}) is of this form.

Next we use (\ref{identAe}) to rewrite (\ref{upe}) in the form
\begin{equation}
u_p(\theta) = \sum_{k=1}^K \sum_{p=0}^{M-1}\sum_{n=1}^{\infty} 4k
e^{-nk(y_k+p\Delta)} \sin{(nk\theta+n\phi_k)} \ . \label{3sume}
\end{equation}
Exchanging order of summation between $n$ and $p$ we can perform the
geometric sum
on $p$. Denoting
\begin{equation}
b_{n,k}\equiv \sum_{p=0}^{M-1}
e^{-nkp\Delta}={1-e^{-Mkn\Delta}\over 1-e^{-kn\Delta}} \ ,
\label{be}
\end{equation}
we find
\begin{eqnarray}
u_p(\theta) &=& \sum_{k=1}^K \sum_{n=1}^{\infty} 4kb_{n,k} e^{-nky_k}
\sin{(nk\theta+n\phi_k)}  \nonumber \\
&=& \sum_{k=1}^K \sum_{n=2}^{\infty} 4kb_{n,k} e^{-nky_k}
\sin{(nk\theta+n\phi_k)} \nonumber \\ &+&\sum_{k=1}^K  4kb_{1,k}
e^{-ky_k} \sin{(k\theta+\phi_k)} \ . \label{2sume}
\end{eqnarray}
Compare now the second term on the RHS of (\ref{2sume}) with
(\ref{Fouriere}). We can identify
\begin{equation}
e^{-ky_k} = {A_k\over 4kb_{1,k}} \label{chooseye}
\end{equation}
The first term can be then bound from above as
\begin{eqnarray}
&&\Big | \sum_{k=1}^K \sum_{n=2}^{\infty} 4kb_{n,k} e^{-nky_k}
\sin{(nk\theta+n\phi_k)}\Big | \label{in1e} \\ &&\le  \sum_{k=1}^K
\sum_{n=2}^{\infty} \Big |4kb_{n,k} \left[{A_k\over
4kb_{1,k}}\right]^n \sin{(nk\theta+n\phi_k)\Big|} \nonumber .
\end{eqnarray}
The sine function and the factor $(4K)^{1-n}$ can be replaced by
unity and we can bound the RHS of (\ref{in1e}) by
\begin{equation}
\sum_{k=1}^K \sum_{n=2}^{\infty}\left[{A_k\over b_{1,k}}\right]^n
b_{n,k} \le \sum_{k=1}^K A_k \sum_{n=1}^{\infty}\left[{A_k\over
b_{1,k}}\right]^n\label{in2e} ,
\end{equation}
where we have used the fact that $b_{n,k}\le b_{1,k}$ which
follows directly from (\ref{be}). Using now the facts that
$b_{1,K}\le b_{1,k}$ for every $k\le K$ and that $A_k$ is bounded
by some finite $C$ since it is a Fourier coefficient, we can bound
(\ref{in2e}) by $C^2K /(b_{1,K}-C)$. Since we can select the free
parameters $\Delta$ and $M$ to make $b_{1,K}$ as large as we want,
we can make the remainder series smaller in absolute value than
$\epsilon/2$.

The conclusion of this demonstration is that any initial condition
that can be represented in Fourier series can be approximated to a
desired accuracy by pole-decomposition. The number of needed poles
is of the order $K^2\times M$. Of course, the number of poles thus
generated by the initial conditions may exceed the number $N(L)$
found in Eq.(\ref{NofLe}). In such a case the excess poles will
move to infinity and will become irrelevant for the short time
dynamics. Thus a smaller number of poles may be needed to describe
the state at larger times than at $t=0$.
 We need to stress at this point that the pole
decomposition is
over complete; for example, if there is exactly one pole at $t=0$ and we use the
above technique to reach a pole decomposition we would get a large number
of poles in our representation.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The initial stages of the front evolution: the exponential stage and
the inverse cascade}

In this section we employ the connection between Fourier expansion and pole
decomposition to understand the initial exponential stage of the evolution of the flame
front with small initial data $u(\theta,t=0)$. Next we employ our knowledge of the pole
interactions  to explain the slow dynamics of coarsening  into the steady state solution.

Suppose that initially the expansion (\ref{Fouriere}) is available
with all the coefficients $A_k\ll 1$. We know from the linear
instability of the flat flame front that each Fourier component
changes exponentially in time according to the linear spectrum
(\ref{spece}). The components with wave vector larger than
(\ref{kmaxe}) decrease, whereas those with lower wave vectors
increase. The fastest growing mode is $k_c=L/2\nu$. In the linear
stage of growth this mode will dominate the shape of the flame
front, i.e.
\begin{equation}
u(\theta,t)\approx A_{k_c}e^{\omega_{k_c}t} \sin(k_c\theta) \ .
\label{initiale}
\end{equation}
Using Eq.(\ref{identCe}) for a large value of $y$ (which is
equivalent to small $A_{k_c}$) we see that to the order of
$O(A^2_{k_c})$ (\ref{initiale}) can be represented as a sum over
$L/2\nu$ poles arranged periodically along the $\theta$ axis.
Other unstable modes will contribute similar arrays of poles but
at much higher values of $y$, since their amplitude is
exponentially smaller. In addition we have nonlinear corrections
to the identification of the modes in terms of poles. These
corrections can be again expanded in terms of Fourier modes, and
again identified with poles, which  will  be further away along
the $y$ axis, and with higher frequencies. To see this one can use
Eq.(\ref{2sume}), subtract from $u_p(\theta)$ the leading pole
representations, and reexpand in Fourier series. Then we identify
the leading order with double the number of poles that are
situated twice further away along the $y$ axis.

We note that even when all the unstable modes are present, the
number of poles in the first order identification is finite for
finite $L$, since there are only $L/\nu$ unstable modes. Counting
the number of poles that each mode introduces we get a total
number of $\Big(L/\nu \Big)^2$ poles. The number $L/2\nu$ of poles
which are associated with the most unstable mode is precisely the
number allowed in the stable stationary solution,
cf.(\ref{NofLe}). When the poles approach the real axis and cusps
begin to develop, the linear analysis no longer holds, but the
pole description does.

We  now describe the qualitative scenario for
the establishment of the steady state. Firstly, we understand that all the
poles that belong to less unstable
modes will be pushed towards infinity. To see this think of the system at
this stage
as an array of uncoupled systems with  a scale of the order of unity. Each such
system will have a characteristic value of $y$. As we discussed
before poles
that are further away along the $y$ axis will be pushed to infinity.
Therefore the system will remain with the $L/2\nu$ poles of the most unstable mode.
The net
effect of the poles belonging to the (nonlinearly) stable modes is to
destroy the otherwise
perfect periodicity of the poles of the unstable mode. The see the effect of the
higher order correction to the pole identification we again recall that they
can be represented as further away poles with higher frequencies, whose dynamics is
similar to the less unstable modes that were just discussed. They do not become more
relevant when time goes on.

Once the poles of the
stable modes get sufficiently far from the real axis, the
dynamics of the  remaining poles will begin to develop according to the interactions
that are directed along the real axis.
These interactions are much weaker and the resulting dynamics occur on much longer time
scales.
The qualitative picture is of an inverse cascade of merging the $\theta$
positions of the poles.
We  note that the system has a set of unstable fixed points which are 'cellular solutions'
 described by a periodic arrangement of
poles along the real axis with a frequency $k$.  These fixed points are not stable
and they collapse,
under perturbations, with a characteristic time scale (that depends on $k$)
to  the next unstable  fixed point
at $k'=k/2$. This process then goes on indefinitely until
$k \sim1/L$ i.e. we reach the  giant cusp, the steady-state stable solution \cite {coars}.

This scenario is seen very clearly in the numerical simulations. In Fig.2.3 we show
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
%\epsfxsize=9.0truecm
%\epsfbox{Fir7.ps}
\psfig{file=fig3.ps,width=7.0cm,angle=-90} \caption { The inverse
cascade process of coarsening that occurs after preparing the
system with random, small initial conditions. One sees that at
successive times the typical scale increases until the giant cusp
forms, and attracts all the other side-poles. The effect of the
existing numerical additive noise is to introduce poles that
appear as side cusps that are continuously attracted to the giant
cusp. This effect is obvious to the eye only after the typical
scale is sufficiently large, as is seen in the last time (see text
for further details).} \label{file=Fig.1e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

the time evolution of the flame front starting from small white-noise initial
conditions. The bottom curve pertains to the earliest time in this picture,
just after
the fast exponential growth, and one sees clearly the periodic array of
cusps that form. The successive images show the progress of the flame front
in time, and
one observes the development of larger scales with deeper cusps that
represent the
partial coalescence of poles onto the same $\theta$ positions. In Fig.2.4
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
%\epsfxsize=9.0truecm
%\epsfbox{Fir7.ps}
\psfig{file=fig4.ps,width=7.0cm,angle=-90}
\caption
{ log-log plots of the front velocity (lower curve) and width (upper
curve)
as a function of time in the inverse cascade process seen in Fig.2.3 in a system o
f size
$2000$ and $\nu=1$.
 Both quantities
 exhibit an initial exponential growth that turns to a power law growth (after
 $t\approx 30$). The velocity is constant after this time, and the width
 increases
 like $t^\zeta$. Note that at the earliest time there is a slight decrease
 in the
 velocity; this is due to the decay of linearly stable modes that exist in random
 initial conditions.}
\label{file=Fig.1e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

we
show the
width and the velocity of this front as a function of
time. One recognizes the exponential stage of growth in which the $L/2\nu$
poles
approach the $\theta$ axis, and then a clear cross-over to much slower dynamics
in which the effective scale in the system grows with a slower rate.

The slow dynamics stage
can be understood qualitatively using the previous interpretation of the
cascade as follows: if the initial number of poles belonging
to the unstable mode is $L/2\nu$, the initial effective linear scale is
$2\nu$. Thus the
first step of the inverse cascade will be completed in a time scale of the order
of $2\nu$. At this point the effective linear scale doubles to $4\nu$, and
the second
step will be completed after such a time scale. We want to know what is the
typical
length scale $l_t$ seen in the system at time $t$.
The definition of front width is $l_t=\sqrt{{1 \over \tilde L}
\int_0^{\tilde L}
[h(x,t)- {\bar h}]^2dx}$,${\bar h}={1 \over \tilde L}\int_0^{\tilde L}
h(x,t)dx$.
The typical width of the system at this
stage will be proportional to this scale.

Denote the number of cascade steps that took place
until this
scale is achieved by $s_l$. The total time elapsed, $t(l_t)$ is the sum
\begin{equation}
t(l_t) \sim \sum_{i=1}^{s_l} 2^i \ . \label{tLte}
\end{equation}
The geometric sum is dominated by the largest term and we therefore estimate
$t(l_t)\sim l_t$. We conclude
that the  scale and the width   are  linear in the time elapsed from the initial conditions
($l_t\sim t^\zeta,~\zeta=1$). In noiseless simulations we find (see Fig.2.4)
a value of $\zeta$ which is $\zeta\approx 0.95 \pm 0.1$.
%%%%%%%%%%%%%%
\subsection{Inverse cascade in the presence of noise\label{ICPNe}}
An interesting consequence of the discussion in the last section is that the
inverse cascade process is an effective ``clock" that measures the typical
time scales in this system. For future purposes we need to know the typical
time scales when the dynamics is perturbed by random noise. To this aim we
ran simulations following the inverse cascade in the {\it presence} of external
noise. The main result that will be used in later arguments is that now the
appearance of a typical scale $l_t$ occurs not after time $t$, but rather
according to
\begin{equation}
l_t\sim t^{\zeta}\ , \quad \zeta\approx 1.2\pm 0.1\ .
\label{timescalee}
\end{equation}
The numerical confirmation of this law is exhibited in Fig.2.5 .
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
%\epsfxsize=9.0truecm
%\epsfbox{Fir7.ps}
\psfig{file=fig5.ps,width=7.0cm,angle=-90} \caption {The same as
Fig.2.4 but with additive random noise for a system of size
$1000$, $\nu=0.1$ and $ f=10^{-13}$. The velocity does not
saturate now, and the exponent $\zeta$ characterizing the increase
of the width with time changes to $\zeta=1.2 \pm 0.1$. The
velocity increases in time like $t^\gamma$ with $\gamma\approx
0.48 \pm 0.04$.} \label{file=Fig.1e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We also find
that the front velocity in this case increases with time according to
\begin{equation}
v \sim t^\gamma \ , \quad \gamma\approx 0.48\pm 0.05\ .
\label{defgammae}
\end{equation}
This result will be related to the acceleration of the flame front in noisy
simulations, as will be seen in the next Sections.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%























\section{Acceleration of the Flame Front, Pole Dynamics and Noise}
\label{noisee} A major motivation of this Section is the
observation that in radial geometry the same equation of motion
shows an acceleration of the flame front. The aim of this section
is to argue that this phenomenon is caused by the noisy generation
of new poles. Moreover, it is our contention that a great deal can
be learned about the acceleration in radial geometry by
considering the effect of noise in channel growth. In Ref.
\cite{85TFH} it was shown that any initial condition which is
represented in poles goes to a unique stationary state which is
the giant cusp which propagates with a constant velocity $v=1/2$
up to small $1/L$ corrections. In light of our discussion of the
last section we expect that any smooth enough initial condition
will go to the same stationary state. Thus if there is no noise in
the dynamics of a finite channel, no acceleration of the flame
front is possible. What happens if we add noise to the system?

For concreteness we introduce an additive white-noise term
$\eta(\theta,t)$to the equation of motion  (\ref{eqfinale})  where
\begin{equation}
\eta(\theta,t) = \sum_k{\eta_k(t) \exp{(ik\theta)}}\ ,
\label{etae}
\end{equation}
and the Fourier amplitudes $\eta_k$ are correlated according to
\begin{equation}
<\eta_k(t)\eta^{*}_{k'}(t')>={f \over L} \delta_{k,k'}\delta(t-t')
\ . \label{corre}
\end{equation}
We will first examine the result of numerical simulations of noise-driven
dynamics,
and later return to the theoretical analysis.
%%%%%%%%%%%%%%%%%%%%%%
\subsection{Noisy Simulations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{bfig1.ps} \caption {The dependence
of the average velocity $v$ on the system size $L$ for $f^{0.5}=0,
2.7\times  10^{-6}, 2.7\times 10^{-5}, 2.7\times 10^{-4},
2.7\times 10^{-3}, 2.7\times 10^{-2}, 2.7\times 10^{-1}, 0.5, 1.3,
2.7$.} \label{file=Fig.2e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{bfig2.ps} \caption {The dependence
of the average velocity $v$ on the noise $f^{0.5}$ for L=10, 40,
80.} \label{file=Fig.2e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Previous numerical  investigations \cite{94FSF,90GS} did not
introduce noise in a controlled fashion. We will argue later that
some of the phenomena encountered in these simulations can be
ascribed to the (uncontrolled) numerical noise. We performed
numerical simulations of Eq.(\ref{eqfinale} using a
pseudo-spectral method. The time-stepping scheme was chosen as
Adams-Bashforth with 2nd order precision in time. The additive
white noise was generated in Fourier-space by choosing $\eta_k$
for every $k$ from a flat distribution in the interval
$[-\sqrt{2{f \over L}},\sqrt{2{f \over L}}]$. We examined the
average steady state velocity of the front as a function of $L$
for fixed $f$ and as a function of $f$ for fixed $L$. We found the
interesting phenomena that are summarized here:
\begin{enumerate}
\item
In Fig.2.7 we can see two different regimes of the   behavior of
the average velocity
$v$ as a  function of the noise
$f^{0.5}$ for the fixed system size L. For the noise $f$ smaller then same fixed value
$f_{cr}$
\begin{equation}
v\sim f^\xi \ . \label{vfe}
\end{equation}
For these values of $f$ this dependence is very weak, and
$\xi\approx 0.02$.
 For the
 large values of $f$ the dependence is much stronger
\item
In Fig.2.6 we can see the growth of the average velocity $v$ as a function of
the system size L. After some values of L we can see saturation of the
velocity.
For regime $f<f_{cr}$ the growth of the velocity can be written as
\begin{equation}
v\sim L^\mu , \quad \mu\approx 0.35\pm 0.03 \ . \label{scale1e}
\end{equation}
\item
In Fig.2.8 and Fig.2.9 we can see flame fronts for $f<f_{cr}$ and
$f>f_{cr}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
%\epsfxsize=9.0truecm
%\epsfbox{fig9.ps}
\psfig{file=fig9.ps,width=7.0cm,angle=-90} \caption {Typical flame
fronts for $f<f_{cr}$  where the system is sufficiently small not
to be terribly affected by the noise. The effect of noise in this
regime is to add additional small cusps to the giant cusp. In
figures a-d we present
 fronts for growing system sizes  $\tilde L=10,20,40$ and $80$ respectively,
 $\nu = 0.1$ .
  One can observe that when
  the system size grows there are more cusps with a more complex structure.}
\label{file=Fig.1e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
%\epsfxsize=9.0truecm
%\epsfbox{Fir7.ps}
\psfig{file=fig10.ps,width=7.0cm,angle=-90}
\caption
{A typical flame front for $f>f_{cr}$. The system size is $160$.
  This is sufficient to cause a
 qualitative change in the appearance of the flame front: the noise introduces
 significant levels of small scales structure in addition to the cusps.}
\label{file=Fig.1e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Calculation  of the Number of Poles in the System}
The interesting problem that we would like to solve here to better
understand the dynamics of poles, is to determine those that exist
in our system outside the giant cusp. This can be done by
calculating  the number of cusps (points of minimum or
inflectional points) and their position on the interval $
\theta:[0,2\pi]$ in every moment of time and  drawing the
positions of the cusps like functions of time, see Fig. 2.10. In
this picture we can see the x-positions of all cusps in the system
as a function of time.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{fbar3.ps} \caption {The dependence
of the cusps positions  on time. $L=80$ $\nu=0.1$ $f=9\times
10^{-6}$} \label{file=Fig.2e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We have assumed that our system is
in a  ``quasi-stable" state most of the time, i.e. every new cusp that
appears in
the system includes only one pole.
Using pictures obtained in this way we can find:
\begin{enumerate}
\item The mean number of poles in the system. By  calculating the
number of cusps in some moment of time and
by investigating  the history of every cusp (except the giant cusp),
 i.e. how many initial cusps
take part in formatting this cusp, and  after averaging the number
of poles found with respect to different moments of time, we can
find  the mean number of poles that exist  in our system outside
the giant cusp. Let us denote this number by $\delta N$. There are
four regimes that can be defined with respect to the dependence of
this number on the noise $f$:

(i) Regime I: Such little noise that
no new cusps exist in our system outside the giant cusp;

(ii)
Regime II: Strong dependence of the pole number  $\delta N$  on the noise $f$;

(iii) Regime III: Saturation  of the pole number  $\delta N$  on the noise $f$,
so  that this number depends very little on the noise (Fig. 2.12);


\begin{equation}
\delta N \sim   f^{0.03}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{fl1.ps} \caption {The dependence of
the pole number in the unit time $dN/dt$ on the noise $f^{0.5}$.
$\nu=0.1$ $ L=80$} \label{file=Fig.2e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{fl2.ps} \caption {The dependence of
the excess pole number $\delta N$ on the noise $f^{0.5}$.
$\nu=0.1$ $ L=40,80$.} \label{file=Fig.2e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{fl3.ps} \caption {The dependence of
the pole number in the unit time $dN/dt$ on the system size L.
$\nu=0.1$ $ f^{0.5}=9\times 10^{-6}$.} \label{file=Fig.2e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{fl4.ps} \caption {The dependence of
the excess pole number $\delta N$  on the system size L. $\nu=0.1$
$ f^{0.5}=9\times 10^{-6}$} \label{file=Fig.2e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{fl5.ps} \caption {The dependence of
the pole number in the unit time  $dN/dt$ on the parameter $\nu$.
$L=80$ $ \nu=0.1$.} \label{file=Fig.2e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{fl6.ps} \caption {The dependence of
the excess pole number $\delta N$  on the the parameter $\nu$.
$L=80$ $ \nu=0.1$.} \label{file=Fig.2e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The saturated value of $\delta N$ is defined by next formula (Fig. 2.14,
Fig. 2.16)

\begin{equation}
\delta N \approx   N(L)/2 \approx {1 \over 4} {L \over \nu} \,
\end{equation}

where $N(L) \approx {1 \over 2} {L \over \nu}$ is the number of poles in
the giant
cusp.

(iv) Regime IV: We again see a strong dependence of the pole number  $\delta N$
on the noise $f$ (Fig. 2.12);

\begin{equation}
\delta N \sim   f^{0.1}
\end{equation}

Because of the numerical noise we can see in most of the simulations only
regime III
and IV. In the future if no new evidence is seen we will discuss regime III.

\item By calculating the new cusp number that appears in the system in the
unit time we can find the number of poles
that appear in the system in the unit  time ${ dN \over dt}$.
In regime III (Fig. 2.11)

\begin{equation}
{ dN \over dt} \sim   f^{0.03}
\end{equation}

The dependence on $L$ and $\nu$ is defined by (Fig. 2.13  and Fig. 2.15)

\begin{equation}
{ dN \over dt} \sim  L^{0.8}
\end{equation}


\begin{equation}
{ dN \over dt} \sim  {1 \over \nu^2}
\end{equation}

In regime IV, the dependence on the noise is defined by the following:
(Fig. 2.11)

\begin{equation}
{ dN \over dt} \sim   f^{0.1}
\end{equation}
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Theoretical Discussion of the Effect of Noise}
\subsubsection{The Threshold of Instability to Added Noise. Transition
from regime I to regime II} \label{regime0e} First we present the
theoretical arguments that explain the sensitivity of the giant
cusp solution to the effect of added noise. This sensitivity
increases dramatically with increasing the system size $L$. To see
this we use again the relationship between the linear stability
analysis and the pole dynamics.

Our additive noise introduces perturbations with all $k$-vectors. We showed
previously
that the most unstable mode is the $k=1$ component $A_1 \sin(\theta)$. Thus the
most effective noisy perturbation is $\eta_1 \sin(\theta)$ which can
potentially lead
to a growth of the most unstable mode. Whether or not this mode will grow
depends
on the amplitude of the noise. To see this clearly we return to the pole
description.
For small values of the amplitude $A_1$ we represent $A_1 \sin(\theta)$ as a
single
pole solution of the functional form $\nu e^{-y}\sin{\theta}$. The $y$
position is
determined from $y=-\log{|A_1| /\nu}$, and the $\theta$-position is
$\theta=\pi$ for
positive $A_1$ and $\theta=0$ for negative $A_1$. From the analysis of
Section III we know that
for very small $A_1$ the fate of the pole is to be pushed to infinity,
independently
of its $\theta$ position; the dynamics is symmetric in $A_1\to -A_1$ when $y$ is
large enough. On the other hand when the value of $A_1$ increases the symmetry
is broken and the $\theta$ position and
the sign of $A_1$ become very important. If $A_1>0$ there is a threshold value
of $y$ below which the
pole is attracted down. On the other hand if $A_1<0$, and $\theta=0$ the
repulsion
from the poles of the giant cusp grows with decreasing $y$. We thus
understand that
qualitatively speaking the dynamics of $A_1$ is characterized by an asymmetric
``potential" according to
\begin{eqnarray}
\dot A_1 &=& -{\partial V(A_1)\over \partial A_1}\ , \label{dvdae}\\
V(A_1) &=& \lambda A_1^2 -aA_1^3+\dots \ . \label{potene}
\end{eqnarray}
>From the linear stability analysis we know that $\lambda\approx \nu/L^2$,
cf. Eq.(\ref{yae}). We know further that the threshold for
nonlinear instability is at $A_1\approx \nu^3/L^2$, cf.
Eq(\ref{nu3L2e}). This determines that value of the coefficient
$a\approx 2/3\nu^2$. The magnitude of the ``potential" at the
maximum is
\begin{equation}
V(A_{max}) \approx \nu^7/L^6 \ . \label{vmaxe}
\end{equation}
The effect of the noise on the development of the mode $A_1\sin{\theta}$ can be
understood from the following stochastic equation
\begin{equation}
\dot A_1 = -{\partial V(A_1)\over \partial A_1}+\eta_1(t) \ .
\label{stochAe}
\end{equation}
It is well known \cite{Ris} that for such dynamics the rate of escape $R$
over the ``potential" barrier
for small noise is proportional to
\begin{equation}
R\sim {\nu\over L^2} \exp^{-\nu^7/{f }L^5} \ . \label{wowe}
\end{equation}
The conclusion is that any arbitrarily tiny noise becomes effective when the
system size increase and when $\nu$ decreases. If we drive the system with noise
of amplitude ${f \over L}$ the system can always be sensitive to this noise when its size
exceeds a critical value $L_c$ that is determined by ${f/ L_c} \sim \nu^7/L_c^6$.
This formula defines transition from regime I (no new cusps) to regime II.
For $L>L_c$
the noise will introduce new poles into the system.
Even numerical noise in simulations involving large size systems may have
a macroscopic influence.

The appearance of new poles must increase the velocity of the
front. The velocity is proportional to the mean of $(u/L)^2$. New
poles distort the giant cusp by additional smaller cusps on the
wings of the giant cusp, increasing $u^2$. Upon increasing the
noise amplitude more and more smaller cusps appear in the front,
and inevitably the velocity increases. This phenomenon is
discussed quantitatively in Section \ref{noisee}.
%%%%%%%%%%%%%%%%%%
\subsubsection{Numerical verifying  of the
asymmetric ``potential" form and dependence of
the noise on $L_c$}
From the equations of the motion for poles we can find the distribution of poles
in the giant cusp \cite{85TFH}.
If we know the distribution of poles in the giant cusp we can then find the form of the
``potential" and verify numerically expressions for values $\lambda$, $A_{max}$
and
${\partial V(A_1) \over \partial A_1}$  discussed previously. The
connection between amplitude $A_1$ and the position of the pole $y$ is defined
by $A_1=4 \nu e^{-y}$ and the connection between the potential function $
{\partial V(A_1) \over \partial A_1}$
and the position of the pole $y$ is defined by formula
${\partial V(A_1) \over \partial A_1}= 4 \nu {dy \over dt} e^{-y}$,
where ${dy \over dt}$ can be determined from the equation of the motion of
the poles.
We can find $A_{max}$ as the
zero-point of ${\partial V(A_1) \over \partial A_1}$
and $\lambda$ can be found as ${1 \over 2}
{\partial^2 V(A_1) \over \partial A_1^2}$ for $A_1=0$.
Numerical measurements were made for the set of values $ L=2 n \nu$,
where $n$ is a integer and $ n>2$.
For our numerical measurements we use  the constant $\nu=0.005$ and the
variable $L$, where
$L$ changes in the interval [1,150], or
 variable $\nu$ that changes in the interval [0.005,0.05] and the
 constant $L=1$.
The  results obtained follow:
\begin{enumerate}
\item
${ A_{max} L^2 \over \nu^3}$ as a function of $L$ is almost a constant.
(Fig. 2.17)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{ff1.ps} \caption {The dependence of
the  normalized amplitude $A_{max}L^2/\nu^3$ on the system size
$L$.} \label{file=Fig.1e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item
${ A_{max} L^2 \over \nu^3}$ as a function of $\nu$ is almost a constant.
(Fig. 2.18)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{ff2.ps} \caption {The dependence of
the  normalized amplitude $A_{max}L^2/\nu^3$ on the parameter
$\nu$.} \label{file=Fig.1e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item
  ${A_{max} \over A_{N(L)}}$
as a function of $L$ is almost a constant.
($A_{N(L)}$ is defined by the position of the upper pole.)
(Fig. 2.19)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{ff3.ps} \caption {The relationship
between the amplitude defined by the minimum of the potential
$A_{max}$ and the amplitude defined by the position of the upper
pole $A_{N(L)}$ as a function of the system size $L$.}
\label{file=Fig.1e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item
${A_{max} \over A_{N(L)}}$ as a function of $\nu$ is almost a constant.
(Fig. 2.20)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{ff4.ps} \caption {The relationship
between the amplitude defined by the minimum of the potential
$A_{max}$ and the amplitude defined by the position of the upper
pole $A_{N(L)}$ as a function of the parameter $\nu$.}
\label{file=Fig.1e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item
The value of ${\lambda L^2 \over \nu}$ as a function of $L$ is a constant
(Fig. 2.21).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{ff5.ps} \caption {The dependence of
the  normalized parameter $\lambda L^2/\nu$ on the system size
$L$.} \label{file=Fig.1e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item
The value of ${\lambda L^2 \over \nu}$ as a function of $\nu$ is  a constant
( Fig. 2.22 ).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm
\epsfbox{ff6.ps}
\caption
{The dependence of the  normalized parameter $\lambda L^2/\nu$
on the parameter $\nu$.}

\label{file=Fig.1e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{bfig3.ps} \caption {The dependence
of the critical noise on the system size.} \label{file=Fig.2e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{enumerate}
We also verify the boundary between regime I (no new cusps) and
regime II (new cusps appear).
Fig. 2.23 shows the  dependence of ${f \over L_c}$
on $L_c$. We can see that ${f/ L_c} \sim 1/L_c^6$.
These results are in good agreement with the theory.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{The Noisy Steady State and its Collapse with
Large Noise and System Size} In this subsection we discuss the
response of the giant cusp solution to noise levels that are able
to introduce a large number of excess poles in addition to those
existing in the giant cusp. We will denote the excess number of
poles by $\delta N$. The first question that we address is how
difficult is it to insert yet an additional pole when there is
already a given excess $\delta N$. To this aim we estimate the
effective potential $V_{\delta N}(A_1)$ which is similar to
(\ref{potene}) but is taking into account the existence of an
excess number of poles. A basic approximation that we employ is
that the fundamental form of the giant cusp solution is not
seriously modified by the existence of an excess number of poles.
Of course this approximation breaks down quantitatively already
with one excess pole. Qualitatively however it holds well until
the excess number of poles is of the order of the original number
$N(L)$ of the giant cusp solution. Another approximation is that
the rest of the linear modes play no role in this case. At this
point we limit the discussion therefore to the situation $\delta
N\ll N(L)$ (regime II).

To estimate the parameter $\lambda$ in the effective potential we
consider the dynamics of one pole whose $y$ position $y_a$ is far
above $y_{max}$. According to Eq.(\ref{yae}) the dynamics reads
\begin{equation}
{dy_a\over dt}\approx {2\nu (N(L)+\delta N)\over L^2} -{1\over L}
\end{equation}
Since the $N(L)$ term cancels against the $L^{-1}$ term (cf. Sec. II A),
we remain
with a repulsive term that in the effective potential translates to
\begin{equation}
\lambda={\nu\delta N\over L^2} \ . \label{lambda2e}
\end{equation}
Next we estimate the value of the potential at the break-even
point between attraction and repulsion. In the last subsection we
saw that a foreign pole has to be inserted below $y_{max}$ in
order to be attracted towards the real axis. Now we need to push
the new pole below the position of the existing  pole whose index
is $N(L)-\delta N$. This position is estimated as in Sec III C by
employing the TFH distribution function (\ref{diste}). We find
\begin{equation}
y_{\delta N}\approx 2\ln{\Big[{4L\over \pi^2\nu\delta N}\Big]} \ .
\label{ydelNe}
\end{equation}
As before, this implies a threshold value of the amplitude of single pole
solution
$A_{max}\sin{\theta}$ which is obtained from equating $A_{max}=\nu
e^{-y_{\delta N}}$.
We thus find in the present case $A_{max}\sim \nu^3(\delta N)^2/L^2$. Using
again
a cubic representation for the effective potential we find $a=2/(3\nu^2\delta
N)$ and
\begin{equation}
V(A_{max}) = {1\over 3}{\nu^7(\delta N)^5\over L^6}\ .
\label{max2e}
\end{equation}
Repeating the calculation of the escape rate over the potential barrier we find
in the present case
\begin{equation}
R\sim {\nu\delta N\over L^2} \exp^{-\nu^7(\delta N)^5/{f  }L^5} \
. \label{wow2e}
\end{equation}

For a given noise amplitude ${f }$ there is always a value of $L$ and $\nu$ for
which
the escape rate is of $O(1)$ as long as $\delta N$ is not too large. When
$\delta N$
increases the escape rate decreases, and eventually no additional poles can
creep
into the system. The typical number $\delta N$ for fixed values of the
parameters is
estimated from equating the argument in the exponent to unity
\begin{equation}
\delta N\approx \left({f }L^5/\nu^7\right)^{1/5} \ .
\label{deltaNe}
\end{equation}

We can see that $\delta N$ is strongly dependent on noise $f$,
in contrast to regime III. Let us find the conditions of transition
from regime II to III, where we see the saturation of $\delta N$
with respect to noise $f$.

(i)  We use the expression $A_{max}=4 \nu  e^{-y_{\delta N}}$
for the amplitude of the pole solution that
equals to ${2\nu \sin \theta \over \cosh(y_{\delta N}) - \cos \theta }$;
 however, this is correct  only for the large number $y_{\delta N}$. When
$y_{\delta N} < 1 $, a better approximation is $A_{max}= {4 \nu
\over y_{\delta N}^2}$. From the equation (\ref{ydelNe}) we find
that the boundary value $y_{\delta N}=1$ corresponds to $\delta N
\approx N(L)/2$.

(ii) We use  the expression $y_{\delta N} \approx
2\ln{\Big[{4L\over \pi^2\nu\delta N}\Big]}$, but for a large value of
$\delta N$ a better approximation that can be found the same way is
$y_{\delta N} \approx {\pi^2 \nu \over 2 L}(N(L)-\delta N)
\ln {\Big[{ 8eL \over \pi^2 \nu (N(L)-\delta N)}\Big]}$ \cite{85TFH}.
These expressions give us  nearly lthe same result for
$\delta N \approx N(L)/2$.

From (i) and (ii) we can make the following conclusions:

(a) The transition from regime II to regime III generally occurs for
$\delta N \approx N(L)/2$;

(b) Using the new expressions in (i) and (ii) for the amplitude $A_{max}$ and
$y_{\delta N}$, we can determine the noise ${f \over L}$ in regime III by

\begin{equation}
{f \over L} \sim V(A_{max}) \sim \lambda A_{max}^2 \sim {\nu \delta N \over
L^2} ({4\nu \over y_{\delta N}^2})^2 \sim {L^2 \over \nu}  {\delta N
\over (N(L)-\delta N)^4}
\end{equation}

This expression defines a very slight dependence of $\delta N$ on the
noise ${f }$
for $\delta N > N(L)/2$, which explains the  noise saturation of $\delta N$
for regime III.

(c) The form of the giant cusp solution is governed by the poles that are
close to zero with respect to $y$.
For the regime III, $N(L)/2$ poles that have positions
$y < y_{\delta N=N(L)/2}=1$ remain at this position. This result explains
why the giant cusp solution cannot be seriously modified for regime III.

From eq. (\ref{deltaNe}) by using the  condition
\begin{equation}
\delta N \approx N(L)/2\, \label{pollae}
\end{equation}
the boundary noise $f_b$ between regimes II and III can be found as

\begin{equation}
f_b \sim { \nu^2 } \ . \label{nosee}
\end{equation}

The basic equation describing pole dynamics follows

\begin{equation}
{dN \over dt}={\delta N \over T} \ , \label{tlif1e}
\end{equation}

where ${dN \over dt}$ is the number of poles that appear in the unit time
in our system, $\delta N$ is the excess number of poles, and T is the mean
lifetime of a pole
 (between appearing and merging with the giant cusp). Using the result
 of numerical
simulations for ${dN \over dt}$ and (\ref{pollae}) we can find for
$T$

\begin{equation}
T = {\delta N \over {dN \over dt}} \sim \nu L^{0.2} \ .
\label{tlife}
\end{equation}


Thus the lifetime is proportional to $\nu$ and depends on the system size $L$
very slightly.


Moreover, the lifetime of a pole is defined by the lifetime of the
poles that are in a cusp. From the maximum point of the linear
part of Eq.(\ref{Eqnondime} ), we can find the mean character size
(Fig.9(\cite{jula2}))

\begin{equation}
\lambda_m \sim \nu
\end{equation}

that defines the  size of our cusps. The mean number of poles in a cusp

\begin{equation}
n_{big} \approx {\lambda_m \over 2 \nu} \sim const
\end{equation}

does not
depend on $L$ and $\nu$. The mean  number of cusps is

\begin{equation}
N_{big} \sim
{\delta N \over n_{big}} \sim {L \over \nu} \ .
\end{equation}

Let us assume that some  cusp exists in the main minimum of the system.
 The lifetime of a pole in such a cusp is defined by three parts.

(I) Time of the cusp formation. This time is proportional to the cusp
size (with $\ln$-corrections) and the pole number in the cusp
(from pole motion equations)

\begin{equation}
T_1 \sim \lambda_m n_{big} \sim \nu
\end{equation}

(II) Time that the cusp is in the minimum neighborhood. This time is defined by

\begin{equation}
T_2 \sim {a \over v} \,
\end{equation}

where $a$ is a  neighborhood of minimum, such that the force from the giant cusp
is smaller than the force from the fluctuations of
the excess pole number $\delta N$, and
$v$ is the velocity of a pole in this neighborhood. Fluctuations of excess pole
number $\delta N$ are expressed as


\begin{equation}
N_{fl}=\sqrt{\delta N} \ .
\end{equation}

From this result and the pole motion equations we find that

\begin{equation}
v \sim {\nu \over L} N_{fl} \sim {\nu \over L} \sqrt{{L \over \nu}}
\sim \sqrt{{\nu  \over L}} \ .
\end{equation}

The velocity from the giant cusp is defined by

\begin{equation}
v \sim {\nu \over L} N(L) {a \over L}  \sim {a \over L} \ .
\end{equation}

So from  equating these two equations we obtain

\begin{equation}
a \sim \sqrt{ \nu L}  \ .
\end{equation}

Thus for $T_2$ we obtain

\begin{equation}
T_2 \sim {a \over v} \sim L \ .
\end{equation}

(III) Time of attraction to the giant cusp. From the equations of motion
for the poles we get

\begin{equation}
T_3 \sim L \ln ({L \over a}) \sim L \ln \sqrt{L} \sim L \ .
\end{equation}

The investigated domain of the system size was found to be

\begin{equation}
T_1 \gg T_2,T_3
\end{equation}

Therefore full lifetime is

\begin{equation}
T=T_1 +T_2 +T_3 \sim \nu + s L \ ,
\end{equation}


where $s$ is a constant and

    \begin{equation}
    0 < s \ll 1 \ .
    \end{equation}

This result qualitatively and partly quantatively explains
dependence (\ref{tlife}). From (\ref{tlife}), (\ref{tlif1e}),
(\ref{pollae}) we can see that in regime III   ${dN \over dt}$ is
saturated with the system size $L$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The acceleration of the flame front because of noise}
In this section we estimate the scaling exponents that
characterize the velocity of the flame front as a function of the
system size. To estimate the velocity of the flame front we need
to create an equation for the mean of $<dh/dt>$ given an arbitrary
number $N$ of poles in the system. This equation follows directly
from (\ref{Eqdime})
\begin{equation}
\left<{dh\over dt}\right>={1  \over L^2}{1 \over
2\pi}\int_{0}^{2\pi}u^2d\theta  \ . \label{eqr0e}
\end{equation}
After substitution of (\ref{upolese}) in (\ref{eqr0e}) we get,
using (\ref{xje}) and (\ref{yje})
\begin{equation}
\left<{dh\over dt}\right>=2\nu\sum_{k=1}^N {dy_k\over dt}+2\left( {\nu N\over
     L}-{\nu^2 N^2\over L^2}\right)  \ . \label{r0polee}
\end{equation}
Estimating the second and third terms in this equation are
straightforward.
Writing $N=N(L)+\delta N(L)$ and remembering that $N(L) \sim L/\nu $
and $\delta N(L) \sim N(L)/2$,
we find that
these terms contribute $O(1)$. The first term
 contributes
only when the current of the poles is asymmetric. Noise introduces poles
at a finite
value of $y_{min}$, whereas the rejected poles stream towards infinity
and disappear at the boundary of nonlinearity defined by the
position of the highest pole as

\begin{equation}
y_{max}\approx 2\ln{\Big[{4L\over \pi^2\nu}\Big]} \ .
\label{delNe}
\end{equation}

Thus we have
an asymmetry that contributes to the velocity of the front.
To estimate the first
term let us define

\begin{equation}
d(\sum {dy_k\over dt})=\sum_{l}^{l+dl} {dy_k\over dt} \ ,
\end{equation}

where $\sum_{l}^{l+dl} {dy_k\over dt}$ is the sum over the
poles that are on the
interval $y:[l,l+dl]$.
We can write

\begin{equation}
d(\sum {dy_k\over dt})=d(\sum {dy_k\over dt})_{up}+
d(\sum {dy_k\over dt})_{down} \ ,
\end{equation}

where $d(\sum {dy_k\over dt})_{up}$ is the flux of poles moving up and
$d(\sum {dy_k\over dt})_{down}$ is the flux of poles moving down.

For these fluxes we can write

\begin{equation}
d(\sum {dy_k\over dt})_{up}, -d(\sum {dy_k\over dt})_{down} \leq {dN \over
dt} dl \ .
\end{equation}

So for the first term

\begin{eqnarray}
&&0 \leq \sum_{k=1}^{N} {dy_k\over dt}=
\int_{y_{min}}^{y_{max}}{d(\sum {dy_k\over dt})
\over dl} dl\\ \nonumber &&
=\int_{y_{min}}^{y_{max}}{d(\sum {dy_k\over dt})_{up}+
d(\sum {dy_k\over dt})_{down} \over dl} dl \\ \nonumber &&
\leq {dN \over dt}(y_{max}-
y_{min})\\ \nonumber &&
\leq {dN \over dt}y_{max}
\end{eqnarray}

 Because of slight ($\ln$) dependence of $y_{max}$ on $L$ and $\nu$,
 ${dN \over dt}$ term determines order of nonlinearity for the first term
 in eq (\ref{r0polee}).
 This term equals zero for the symmetric current of poles and achieves the
 maximum
 for the maximal asymmetric current of poles.
 A comparison of $v \sim L^{0.42}f^{0.02}$
 and ${dN \over dt} \sim L^{0.8}f^{0.03}$ confirms this calculation.



















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Summary and Conclusions}

The main two messages of this chapter are: (i) There is an important
interaction between
the instability of developing fronts and random noise; (ii) This
interaction and its
implications can be understood qualitatively and sometimes quantitatively using
the description in terms of complex poles.

The pole description is natural in this context firstly because it
provides an
exact (and effective) representation of the steady state without noise.
Once one succeeds
to describe also the {\em perturbations} about this steady state in terms
of poles,
one achieves a particularly transparent language for the study of the
interplay between
noise and instability. This language also allows us to describe in
qualitative and
semi-quantitative terms the inverse cascade process of increasing typical
lengths when
the system relaxes to the steady state from small, random initial conditions.

The main conceptual steps in this chapter are as follows: firstly one
realizes that
the steady state solution, which is characterized by $N(L)$ poles aligned along
the imaginary axis is marginally stable against noise in a periodic array of
$L$ values. For all values of $L$ the steady state is nonlinearly unstable
against noise. The main and foremost effect of noise of a given amplitude $f$ is
to introduce
an excess number of poles $\delta N(L,f)$ into the system. The existence of this
excess number of poles is responsible for the additional wrinkling of the
flame front on top of the giant cusp, and for the observed acceleration of
the flame front.
By considering the noisy appearance of new poles we rationalize the
observed scaling laws as a function of the noise amplitude and the system size.

Theoretically we therefore concentrate on estimating $\delta N(L,f)$.
We note  that some of our consideration are only qualitative. For example,
we estimated $\delta N(L,f)$ by assuming that the giant cusp solution is not
seriously perturbed. On the other hand we find a flux of poles going to
infinity due
to the introduction of poles at finite values of $y$ by the noise. The
existence of poles
spread between $y_{max}$ and infinity {\em is} a significant perturbation of the
giant cusp solution. Thus also the
comparison between the various scaling exponents measured and predicted must be done
with caution; we cannot guarantee that those cases in which our prediction
hit close
to the measurement mean that the theory is quantitative. However we
believe that
our consideration extract the essential ingredients of a correct theory.

The "phase diagram" as a function of $L$ and $f$ in this system
consists of four regimes (in contradiction with our previous
results \cite{OGKP}). In the first one, discussed in Section
\ref{regime0e} , the noise is too small to have any effect on the
giant cusp solution. The second regime (very small excess number
of poles ) can not be observed because of numerical noise and
discussed only theoretically. In the third regime the noise
introduces excess poles that serve to decorate the giant cusp with
side cusps. In this regime we find scaling laws for the velocity
as a function of $L$ and $f$ and we are reasonably successful in
understanding the scaling exponents. In the fourth regime the
noise is large enough to create small scale structures that are
not neatly understood in terms of individual poles. It appears
from our numerics that in this regime the roughening of the flame
front gains a contribution from the the small scale structure in a
way that is reminiscent of {\em stable}, noise driven growth
models like the Kardar-Parisi-Zhang model.




One of our main motivations in this research was to understand the
phenomena observed
in radial geometry with expanding flame fronts.
. We note that many of the insights offered
above
translate immediately to that problem. Indeed, in radial geometry the flame
front
accelerates and cusps multiply and form a hierarchic structure as time
progresses.
Since the radius (and the typical scale) increase in this system all the
time, new
poles will be added to the system even by a vanishingly small noise. The
marginal
stability found above holds also in this case, and the system
will allow the introduction of excess poles as a result of noise. The
results discussed
in Ref.\cite{KOP95}  can be combined with the present insights to provide a theory
of radial growth ( chapter 4).

Finally, the success of this approach in the case of flame propagation
raises hope
that Laplacian growth patterns may be dealt with using similar ideas. A problem
of immediate interest is Laplacian growth in channels, in which a finger
steady-state solution is known to exist. It is documented that the stability
of such a finger solution to noise decreases rapidly with increasing the channel
width. In addition, it is understood that noise brings about additional
geometric
features on top of the finger. There are enough similarities here to indicate
that a careful analysis of the analytic theory may shed as much light on that
problem as on the present one.

\noindent







%\end{document}


==> ole2.tex <==


%%\documentstyle[aps,pre,preprint,epsfmac,floats]{revtex}
%\documentstyle[aps,pre,preprint,epsf]{revtex}
%\documentstyle[aps,pre,twocolum,epsf,psfig]{revtex}
%\begin{document}
%\def\OP {\tensor P}
%\def\B.#1{{\bbox{#1}}}
%\renewcommand{\thesection}{\arabic{section}}
\chapter{Using of Pole Dynamics for Stability Analysis of Flame Fronts: Dynamical Systems Approach in
the Complex Plane}
%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
In this chapter we discuss the stability of steady flame fronts in channel
geometry.
We write shortly about this topic
in chapter 2 (Sec. 2.3) and we want to consider it in detail in this chapter.
Traditionally \cite{Pel,BS,Vic}
one studies stability by considering the linear operator which is obtained
by linearizing the
equations of motion around the steady solution. The eigenfunctions obtained
are {\em delocalized}
and in certain cases are not easy to interpret.
In the case of flame fronts the steady state solution is space dependent
and therefore the
eigenfunctions are very different from simple Fourier modes. We show in
this chapter that a good
understanding of the
nature of the eigenspectrum and eigenmodes can be obtained by doing almost
the opposite
of traditional stability analysis, i.e., studying the {\em localized}
dynamics of
singularities in the complex plane. By reducing the stability analysis to a
study of a finite
dimensional dynamical system one can gain considerable intuitive
understanding of the nature
of the stability problem.

The analysis is based on the understanding that for a given channel width
$L$ the steady state solution for the
flame front is given in terms of $N(L)$ poles that are organized on a line
parallel to the
imaginary axis \cite{85TFH}. Stability of this solution can then be
considered in two
steps. In the
first step we examine the response of this set of $N(L)$ poles to
perturbations in their
positions. This procedure yields an important part of the stability
spectrum. In the second
step we examine general perturbations, which can also be described by the
addition of extra poles to the
system of $N(L)$ poles. The response to these perturbations gives us the
rest of the stability
spectrum; the combinations of these two steps rationalizes all the
qualitative features found by traditional stability analysis.

 In Sec.2 we present the results of traditional linear
stability analysis,
and show the eigenvalues and eigenfunctions that we want to interpret by
using the pole
decomposition. Sec. 3 presents the analysis in terms of complex
singularities, in two steps as discussed above. A summary and discussion
is presented in Sec.4.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Linear Stability Analysis in Channel Geometry}

The standard technique to study the linear stability of the steady solution
is to
perturb it by a
small perturbation $\phi(\theta,t)$: $u(\theta,t) =
u_s(\theta)+\phi(\theta,t)$ .
Linearizing the dynamics for small $\phi$ results in the following equation
of motion
\begin{eqnarray}
{\partial \phi(\theta,t) \over \partial t}&=& {1\over L^2}\Big
[\partial_\theta [u_s(\theta) \phi(\theta,t)] \nonumber \\&+&\nu
\partial_\theta^2\phi(\theta,t)\Big] +{1\over L}I(\phi(\theta,t))
\ . \label{rineare} \end {eqnarray} were the linear operator
contains $u_s(\theta)$ as a coefficient. Accordingly simple
Fourier modes do not diagonalize it. Nevertheless, we proceed to
decompose $\phi(x)$ in Fourier modes according to ,
\begin{eqnarray}
\phi(\theta,t)&=&\sum_{k=-\infty}^{\infty} \hat\phi_k(t)
e^{ik\theta}\label{phie}\\
u_s(\theta)&=&-2{\nu}i\sum_{k=-\infty}^{\infty}
\sum_{j=1}^N sign(k)e^{-\mid k \mid y_j}e^{ik\theta}
\end {eqnarray}
The last equation follows from (\ref{state}) by expanding in a
series of $\sin{k\theta}$. In these sums the discrete $k$ values
run over all the integers. Substituting in Eq.(\ref{rineare}) we
get:
\begin{equation}
{d\hat \phi_k(t) ) \over dt}= \sum _n a_{kn} \hat\phi_n(t)\ , \
\end {equation}
where $a_{kn}$ are entires of an infinite matrix:
\begin{eqnarray}
a_{kk}&=&{\mid k \mid\over L} -{\nu \over L^2} k^2 \ ,
\label{akke}\\ a_{kn} &=&{k\over L^2}sign(k-n)({2\nu} \sum_{j=1}^N
e^{-\mid k-n \mid y_j}) \quad k \neq n \ .
\end {eqnarray}
To solve for the eigenvalues of this matrix we need to truncate it
at some cutoff $k$-vector $k^*$. The scale $k^*$ can be chosen on
the basis of Eq.(\ref{akke}) from which we see that the largest
value of $k$ for which $a_{kk}\ge 0$ is a scale that we denote as
$k_{max}$, which is the integer part of $L/\nu$. We must choose
$k^*>k_{max}$ and test the choice by the convergence of the
eigenvalues. The chosen value of $k^*$ in our numerics was
$4k_{max}$. One should notice that this cutoff limits the number
of eigenvalues, which should be infinite. However the lower
eigenvalues will be well represented. The results for the low
order eigenvalues of the matrix $a_{kn}$ that were obtained from
the converged numerical calculation are presented in Fig.3.1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{Fir1.ps} \caption {A plot of the
first five eigenvalues obtained by diagonalizing the matrix
obtained by traditional stability analysis, against the system
size. The eigenvalues are normalized by $L^2/\nu$. The largest
eigenvalue is zero, which is a Goldstone mode. All the other
eigenvalues are negative except for the second and third that
touch zero periodically. The second and fourth eigenvalues are
represented by a  solid line and the third and fifth eigenvalues
are represented by a dot-dashed line.} \label{file=Fig.1e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The eigenvalues are multiplied by $L^2/\nu$ and are plotted as a
function of $L$. We order the eigenvalues in decreasing order and
denote them as $\lambda_0\ge \lambda_1\ge \lambda_2 \dots$. In
addition to the eigenvalues, the truncated matrix also yields
eigenvectors that we denote as $A^{(\ell)}$. Each such vector has
$k^*$ entries, and we can compute the eigenfunctions
$f^{(\ell)}(\theta)$ of the linear operator (\ref{rineare}), using
(\ref{phie}), as
\begin{equation}
f^{(\ell)}(\theta) \equiv \sum _{-k^*}^{k^*} e^{ik\theta}
A^{(\ell)}_k \ . \label{felle}
\end{equation}
Eq.(\ref {rineare}) does not mix even with odd solutions in
$\theta$, as can be checked by inspection. Consequently the
available solutions have even or odd parity, expandable in either
$\cos$ or $\sin$ functions. The first two nontrivial
eigenfunctions $f^{(1)}(\theta)$ and $f^{(2)}(\theta)$ are shown
in Figs.3.2,3.3.
a%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{Fir2.ps} \caption {The first odd
eigenfunction obtained from traditional stability analysis.}
\label{file=Fig.2e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{Fir3.ps} \caption {The first even
eigenfunction obtained from traditional stability analysis.}
\label{file=Fig.3e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
It is evident that the function in Fig.3.2 is odd around
zero whereas in Fig.3.3 it is even. Similarly we can numerically generate any
other eigenfunction of the linear operator,
but we understand neither the physical significance of these eigenfunction
nor the $L$ dependence of their associated eigenvalues shown in Fig.3.1
In the next section we
will demonstrate how the dynamical system approach in terms of
singularities in the
complex plane provides us with considerable intuition about these issues.
%%%%%%%%%%%%%%%%%%%
\section{Linear Stability in terms of complex singularities} Since the
partial differential equation
is continuous there is an infinite number of modes. To understand this in
terms of pole dynamics we consider
the problem in two steps: First, we consider the $2N(L)$ modes associated
with the dynamics of the
$N(L)$ poles of the giant cusp.
In the second step we explain
that all the additional modes result from the introduction of additional
poles, including
the reaction of the $N(L)$ poles of the giant cusp to the new poles. After
these two steps
we will be able to identify all the linear modes that were found
by diagonalizing the stability matrix in the previous section.
%%%%%%%%%%%%%%%%%
\subsection{The modes associated with the giant cusp} In the steady
solution all the
poles occupy stable equibirilium positions. The forces operating
on any given pole cancel exactly, and we can write matrix equations for
small perturbations
in the pole positions $\delta y_i$ and $\delta x_i$.

Following \cite{85TFH} we rewrite the equations of motion
(\ref{yje}) using the Lyapunov function $U$:
\begin{equation}
L\dot{y_i}={\partial U \over \partial y_i} \label{hil1e}
\end{equation} where ${i=1,...,N}$ and

\begin{eqnarray}
U={\nu \over L}[ \sum_i\ln \sinh y_i&+&2\sum_{i<k} (\ln
\sinh{y_k-y_i \over 2}\nonumber \\&+&\ln \sinh{y_k+y_i \over 2})]
- \sum_iy_i \label{hil2e}
\end{eqnarray}
The linearized equations of motion for $\delta y_i$ are:
\begin{equation} L\dot{\delta y_i}= \sum_k{\partial^2 U \over
\partial y_i \partial y_k }\delta y_k \ . \label{linyje}
\end{equation}
The matrix $\partial^2 U/\partial y_i \partial y_k$ is real and symmetric
of rank $N$.
We thus expect to find $N$ real eigenvalues and N orthogonal eigenvectors.

For the deviations $\delta x_i$ in the $x$ positions we find the following
linearized equations of
motion
\begin{eqnarray}
&&L\dot{\delta x_j}=-{\nu \over L}{\delta x_j} \sum_{k=1, k \neq j}^N
({1 \over \cosh(y_j-y_k)-1)}\nonumber \\ && +{1 \over \cosh(y_j+y_k)-
1}) \nonumber \\ &&+
{\nu \over L} \sum_{k=1, k \neq j}^N {\delta x_k}
({1 \over \cosh(y_j-y_k)-1)}+{1 \over \cosh(y_j+y_k)- 1})
\end{eqnarray}
In shorthand:
\begin{equation}
L{d{\delta x_i}\over dt}=V_{ik}\delta x_k \ . \label{linxie}
\end{equation} The matrix $V$ is also real and symmetric. Thus $V$
and ${\partial^2 U /
\partial y_i \partial y_k}$
together supply $2 N(L)$ real eigenvalues and $2N(L)$ orthogonal
eigenvectors. The explicit form of
the matrices $V$ and ${\partial^2 U / \partial y_i \partial y_k}$ is as follows:
For $i\neq k$:
\begin{equation}
{\partial^2 U \over \partial y_i \partial y_k}= {\nu \over L}[{1/2
\over \sinh^2({y_k-y_i \over 2})}-{1/2 \over\sinh^2({y_k+y_i \over
2})}] \label{mat11e}
\end{equation}

\begin{equation}
V_{ik}={\nu \over L}({1 \over \cosh(y_i-y_k)-1)}+{1 \over
\cosh(y_i+y_k)- 1}) \label{mat12e}
\end{equation}


and for $i=k$ one gets:
\begin{eqnarray}
{\partial^2 U \over \partial y_i^2}= &-&{\nu \over L}[\sum_{k \neq
i}^N \left({1 \over 2\sinh^2({y_k-y_i \over 2})} +{1 \over
2\sinh^2({y_k+y_i \over 2})}\right) \nonumber \\&+&{1 \over
\sinh^2(y_i)}] \label{mat21e}
\end{eqnarray}
\begin{equation}
V_{ii}=\sum_{k \neq i}^N[-{\nu \over L} ({1 \over
\cosh(y_i-y_k)-1)}+{1 \over \cosh(y_i+y_k)- 1})] \label{mat22e}
\end{equation}
Using the known steady state solutions $y_i$ at any given $L$ we can
diagonalize
the $N(L)\times N(L)$ matrices numerically. In  Fig.3.4 we present
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{Fir4.ps} \caption {The eigenvalues
associated with perturbing the positions of the poles that consist
the giant cusp. The largest eigenvalue is zero. The second, third,
fourth and fifth eigenvalues are represented by a solid line,
dot-dashed line, dotted line and dashed line respectively.}
\label{file=Fig.4e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
the eigenvalues of the lowest order
modes obtained from this procedure. The least negative eigenvalues
touch zero periodically. This eigenvalue can be fully identified with the
motion of the highest
pole $y_{N(L)}$ in the giant cusp. At isolated values of $L$ the
position of this pole tends
to infinity, and then the row and the column in our matrices that contain
$y_{N(L)}$ vanish identically, leading to a zero eigenvalue. The rest of the
upper eigenvalues match perfectly with half of the observed eigenvalues in
Fig.3.1. In other words, the eigenvalues observed here agree perfectly
with the ones plotted in this Fig.3.1 until the discontinuous increase
from their minimal points.
The ``second half'' of the oscillation in the eigenvalues as a function of
$L$ is not contained in this spectrum of the $N(L)$ poles of the giant cusp.
To understand the rest
of the spectrum we need to consider perturbation of the giant cusp by
additional poles.
The eigenfunctions can be found using the knowledge of the eigenvectors of
these matrices.
Let us denote the eigenvectors of ${\partial^2 U / \partial y_i \partial
y_k}$ and $V$ as
$a^{(\ell)}$ and $b^{(\ell)}$ respectively. The perturbed solution is
explicitly given as (taken for $x_s=0$): \begin{equation}
u_s(\theta)+\delta u=2\nu \sum_{i=1}^N {\sin(\theta -\delta x_i) \over
\cosh(y_i+\delta y_i)- \cos (\theta -\delta x_i)} \end{equation}
where $\delta u$ is
\begin{eqnarray}
\delta u=&-&4{\nu }\sum_{i=1}^N \sum_{k=1}^{\infty} \delta y_i
ke^{-ky_i}\sin k\theta \nonumber\\ &-&4\nu \sum_{i=1}^N
\sum_{k=1}^{\infty} \delta x_i ke^{-ky_i}\cos k\theta
\label{hil4e}
\end{eqnarray}
So knowing the eigenvectors $a^{(\ell)}$ and $b^{(\ell)}$ we can
estimate the eigenvectors $f^{(\ell)}(\theta)$ of (\ref{felle}):
\begin{equation} f^{(\ell)}_{\rm sin}(\theta) =-4{\nu
}\sum_{i=1}^N \sum_{k=1}^{\infty} a_i^{(j)} k e^{-k y_i}\sin
k\theta \ , \quad j=1,...,N \label{hhh1e}
\end{equation}
or
\begin{equation}
f^{(\ell)}_{\rm cos}(\theta) =-4{\nu }\sum_{i=1}^N
\sum_{k=1}^{\infty} b_i^{(j)} ke^{-ky_i}\cos k\theta\ , \quad
j=1,...,N \label{hhh2e}
\end{equation}
where we display separately the $\sin$ expansion and the $\cos$ expansion.
For the case $j=1$,
the eigenvalue is zero, and a uniform translation of the poles in any
amount $\delta x_i$ results
in a Goldstone mode. This is characterized by an eigenvector $b^{(1)}_i=1$
for all $i$.
The eigenvectors $f^{(\ell)}$ (Fig.3.5,3.6)computed this way are identical to
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{Fir5.ps} \caption {The first odd
eigenfunction associated with perturbing the positions of the
poles in the giant cusp.} \label{file=Fig.5e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{Fir6.ps} \caption {The first even
eigenfunction associated with perturbing the positions of the
poles in the giant cusp.} \label{file=Fig.6e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
numerical
precision with those shown in Figs.3.2,3.3, and observe the agreement.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Modes related to additional poles} In this subsection we
identify the rest of the modes that were not found in the previous
subsection. To this aim we study the response of the TFH solution
to the introduction of additional poles. We choose to add $M$ new
poles all positioned at the same imaginary coordinate $y_p\ll
y_{max}$, distributed at equidistant real positions
$\{x_j=x_0+(2\pi/M)j\}_{j=1}^M$. For $x_0=0$ we use
(\ref{upolese}) and the Fourier expansion  to obtain a
perturbation of the form
\begin{equation}
\delta u(\theta,t) \simeq 4{\nu }M e^{-M y_p (t)}\sin M\theta
\label{hil5e}
\end{equation}
For $x_0=-\pi/2M$ we get
\begin{equation}
\delta u(\theta,t) \simeq 4{\nu }Me^{-My_p (t)}\cos M\theta
\label{hil6e}
\end{equation}
in both cases the equations for the dynamics of $y_p$ follow from
Eqs.(\ref{xje})-(\ref{yje}):
\begin{equation}
{dy_p \over dt} \simeq 2{\nu \over L^2}\alpha(M) \ , \label{dype}
\end{equation} where $\alpha(M)$ is given as:
\begin{equation}
\alpha(M)=[{1 \over 2}({L \over \nu}+1)]-{1 \over 2}({L \over \nu}-M)
\end{equation}
Since (\ref{dype}) is linear, we can solve it and substitute in
Eqs.(\ref{hil5e})-(\ref{hil6e}). Seeking a form $\delta
u(\theta,t)\sim exp(-\lambda(M) t)$ we find that the eigenvalue
$\lambda(M)$ is
\begin{equation}
\lambda(M) =2M{\nu \over L^2}\alpha(M) \label{lamme}
\end{equation}
These eigenvalues are plotted in Fig.3.7
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\narrowtext
\begin{figure}
\epsfxsize=9.0truecm \epsfbox{Fir7.ps} \caption {Spectrum of
eigenvalues associated with the reaction of the poles in the giant
cusp to the addition of new poles.} \label{file=Fig.7e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
At this point we consider the dynamics of the poles in the giant
cusp under the influence of the additional $M$ poles. From
Eqs.(\ref{linyje}), (\ref{linxie}), (\ref{xje}), (\ref{yje}) we
obtain, after some obvious algebra,
\begin{equation}
L\dot{\delta y_i}= \sum_j{\partial^2 U \over \partial y_i \partial y_j
}\delta y_j-4{\nu \over L}Me^{-My_p(t)} \sinh(My_i) \end{equation}
or
\begin{equation}
L\dot{\delta x_i}= \sum_j{V_{ij}
}\delta x_j-4{\nu \over L}Me^{-My_p(t)} \cosh(My_i) \end{equation}
It is convenient now to transform from the basis $\delta y_i$ to the
natural basis
$w_i$ which is obtained using the linear transformation $w =A^{-1}
{\delta y}$.
Here the matrix $A$ has columns which are the eigenvectors of $\partial^2 U
/\partial y_i \partial y_j$
which were computed before. Since the matrix was real symmetric, the matrix
$A$ is
orthogonal, and $A^{-1}=A^T$. Define $C=4{\nu \over L^2}M e^{-M y_p(0)}$
and write
\begin{equation}
\dot{ w_i}=-\lambda_i w_i-Ce^{-\lambda(M) t} \xi_i \ , \label{wie}
\end{equation} where $-\lambda_i$ are the eigenvalues associated
with the columns of $A$, and
\begin{equation}
\xi_i=\sum_j A_{ji}\sinh M y_j \ .
\end{equation}
We are looking now for a solution that decays exponentially at the rate
$\lambda(M)$:
\begin{equation}
w_i(t)=w_{i}(0)e^{-\lambda(M) t}
\end{equation}
Substituting the desired solution in (\ref{wie}) we find a
condition on the initial value of $w_i$:
\begin{equation}
w_{i}(0)=-{C \over \lambda_i- \lambda(M)}\xi_i \end{equation}
Transforming back to $\delta y_i$ we get
\begin{eqnarray}
&&  \delta y_{i}(0)=\sum_k A_{ik}w_{k}(0)=-\sum_k A_{ik} {C \over
\lambda_k- \lambda(M)}\sum_l A_{lk} \sinh M y_l \nonumber \\&&
=-C\sum_l\sinh M y_l \sum_k{A_{ik} A_{lk} \over \lambda_k-
\lambda_p^M} \label{hil7e}
\end{eqnarray}

We can get the eigenfunctions of the linear operator, as before,
using Eqs.(\ref{hil4e}), (\ref{hil5e}), (\ref{hil6e}),
(\ref{hil7e}). We get \begin{eqnarray} &&f^{(M)}_{\rm sin}(\theta)
=4C {\nu }\sum_{i=1}^{N(L)} \sum_{k=1}^{\infty} (\sum_l\sinh M y_l
\sum_m{A_{im} A_{lm} \over \lambda_m- \lambda(M)}) \nonumber \\&&
\times ke^{-ky_i}\sin k\theta+{L^2 }C\sin M\theta \ \label{ril7e}
\end{eqnarray}
An identical calculation to the one started with Eq. (\ref{wie})
can be followed for the deviations $\delta x_i$. The final result
reads \begin{eqnarray} && f^{(M)}_{\rm cos}(\theta) =4C {\nu
}\sum_{i=1}^{N(L)} \sum_{k=1}^{\infty} (\sum_l\cosh My_l
\sum_m{\tilde A_{im} \tilde A_{lm} \over \tilde\lambda_m-
\lambda(M)}) \nonumber \\&& \times ke^{-ky_i}\cos k\theta +{L^2
}C\cos M\theta \ , \label{ril8e}
\end{eqnarray}
where $\tilde A$ is the matrix whose columns are the eigenvectors of $V$,
and $-\tilde \lambda_i$
its eigenvalues.



We are now in position to explain the entire linear spectrum using the
knowledge that we have gained.
The spectrum consists of two separate types of contributions. The first type
has $2N$ modes that belong to the dynamics of the unperturbed $N(L)$ poles
in the giant cusp.
The second part, which is most of the spectrum, is built from modes of the
second type since $M$ can go to infinity. This structure is seen in the
Fig.3.4 and Fig.3.7.

We can argue that the set of eigenfunctions obtained above is
complete and exhaustive. To do this we show that any arbitrary
periodic function of $\theta$ can be expanded in terms of these
eigenfunctions. Start with the standard Fourier series in terms of
sin and cos functions. At this point solve for $\sin{k\theta}$ and
$\cos{k\theta}$ from Eqs.(\ref{ril7e}-\ref{ril8e}). Substitute the
results in the Fourier sums. We now have an expansion in terms of
the eigenmodes $f^{(M)}$ and in terms of the triple sums. The
triple sums however can be expanded, using
Eqs.(\ref{hhh1e}-\ref{hhh2e}), in terms of the eigenfunctions
$f^{(\ell)}$. We can thus decompose any function in terms of the
eigenfunctions $f^{(M)}$ and $f^{(\ell)}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusions}
We discussed the stability of flame fronts in channel geometry
using the representation of the solutions in terms of
singularities in the complex plane. In this language the
stationary solution, which is a giant cusp in configuration space,
is represented by $N(L)$ poles which are organized on a line
parallel to the imaginary axis. We showed that the stability
problem can be understood in terms of two types of perturbations.
The first type is a perturbation in the positions of the poles
that make up the giant cusp. The longitudinal motions of the poles
give rise to odd modes, whereas the transverse motions to even
modes. The eigenvalues associated with these modes are eigenvalues
of a finite, real and symmetric matrices, cf. Eqs.(\ref{mat11e}),
(\ref{mat12e}), (\ref{mat21e}), (\ref{mat22e}). The second type of
perturbations is obtained by adding  poles to the set of $N(L)$
poles representing the giant cusp. The reaction of the latter
poles is again separated into odd and even functions as can be
seen from Eqs.(\ref{hil5e}), (\ref{hil6e}). Together the two types
of perturbations rationalize and explain all the features of the
eigenvalues and eigenfunctions obtained from the standard linear
stability analysis.





%\end{document}


==> oleg3.tex <==


%\documentstyle[aps,prl,twocolumn,epsfmac]{revtex}
%\documentstyle[aps,prl,epsf,twocolumn]{revtex}
%\begin{document}
%\renewcommand{\thesection}{\arabic{section}}
%\draft


\chapter{Dynamics and Wrinkling of Radially Propagating Fronts Inferred from Scaling
Laws in Channel Geometries}
 \section{Introduction}

The main idea of this chapter is that in order to derive scaling laws for
unstable front
propagation in radial geometry, it is useful to study noisy propagation in
channel geometries,
in which the noiseless dynamics results usually in simple shapes of the
advancing fronts \cite{Pel}.

The understanding of radial geometries requires control of the effect of
noise on the
unstable dynamics of propagation. It is particularly difficult to achieve
such a control
in radial geometries due to the vagueness of the distinction between
external noise and noisy
initial conditions. Channel geometries are simpler when they exhibit a
stable solution for
growth in the noiseless limit. One can then study the effects of external
noise in such
geometries without any ambiguity. If one finds rules to translate the
resulting understanding
of the effects of noise in channel growth to radial geometries, one can
derive the scaling laws in the
later situation in a satisfactory manner. We will exemplify the details of
such a translation
in the context of premixed flames that exist as self sustaining fronts of
exothermic chemical
reactions in gaseous combustion. But our contention is that similar ideas
should be fruitful
also in other contexts of unstable front propagation. Needless to say, there
are aspects of the front dynamics and statistics in the radial geometry
that {\em cannot} be explained from observations of fronts in a channel
geometry; examples of such aspects are discussed at the end of this
chapter.

Mathematically our example is described \cite{94FSF} by an equation of
motion for the angle-
dependent modulus of the  radius vector of the flame front,  $R(\theta,t)$:
\begin{eqnarray}
{\partial R \over \partial t}&=&
 {U_b\over 2{R_0}^2(t)}\left({\partial R \over \partial \theta }\right)^2
 +{D_M\over {R_0}^2(t)}{\partial^2 R\over \partial\theta^2}\\ \nonumber &+&
{\gamma
 U_b\over 2R_0 (t)} I(R)+U_b \ . \label{rqdime}
\end{eqnarray}
Here 0$ <\theta <  2\pi$ is an angle and the constants $U_b,D_M$ and
$\gamma$ are the
front velocity for an ideal cylindrical front, the Markstein diffusivity
and the thermal
expansion coefficient respectively. $R_0(t)$ is the mean
radius of the propagating flame:
\begin{equation}
R_0 (t)={1\over 2\pi}\int_{0}^{2\pi}R(\theta,t)d\theta \  .
\label{r0e}
\end{equation}
The functional $I(R)$ is best represented in terms
of its Fourier decomposition. Its Fourier component is $|k|R_k$ where $R_k$
is the
Fourier component of $R$. Simulations of this equation, as well as
experiments in
the parameter regime for which this equation is purportedly relevant,
indicate that for large times $R_0$ grows as a power in time
\begin{equation}
R_0(t) = (const+t)^{\beta} \ , \label{rccele}
\end{equation}
with $\beta>1$, and that the width of the interface $W$
grows with $R_0$ as
\begin{equation}
W(t) \sim R_0(t)^\chi \ , \label{rcalinge}
\end{equation}
with $\chi<1$.




\section{The Geometry of Developing Flame Fronts: Analysis with Pole Decomposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The study of growing fronts in nonlinear physics \cite{Pel} offers
fascinating examples of spontaneous generation of fractal
geometry\cite{BS,Vic}. Advancing fronts rarely remain flat;
usually they form either fractal objects with contorted and
ramified appearance, like Laplacian growth patterns and diffusion
limited aggregates (DLA)\cite{81WS}, or they remain graphs, but
they ``roughen" in the sense of producing self-affine fractals
whose ``width" diverges with the linear scale of the system with
some characteristic exponent. The study of interface growth where
the roughening is caused by the noisy environment, with either
annealed or quenched noise, was a subject of active research in
recent years\cite{93Mea,95HHZ}. These studies met considerable
success and there is significant analytic understanding of the
nature of the universality classes that can be expected. The study
of interface roughening in system in which the flat surface is
inherently unstable is less developed. One interesting example
that attracted attention is the Kuramoto-Sivashinsky equation
\cite{78Kur,77Siv} which is known to roughen in 1+1 dimensions but
is claimed not to roughen in higher dimensions\cite{92LP}. Another
outstanding example is Laplacian growth patterns\cite{84SB}. This
chapter is motivated by a new example of the dynamics of outward
propagating flames whose front wrinkles and fractalizes
\cite{94FSF}. We will see that this problem has many features that
closely resemble Laplacian growth, including the existence of a
single finger in channel growth versus tip splitting in
cylindrical outward growth, extreme sensitivity to noise, etc. In
the case of flame fronts the equation of motion is amenable to
analytic solutions and as a result we can understand some of these
issues.

The physical problem that motivates this analysis is that of pre-mixed
flames which
exist as self-sustaining fronts of exothermic chemical reactions in gaseous
combustion. It had been known for some time that such flames are
intrinsically unstable
\cite{44Lan}.
It was reported that such flames develop characteristic structures which
includes cusps,
and that under usual experimental conditions the flame front accelerates as
time goes
on \cite{89GIS}. In recent work Filyand et al. \cite{94FSF} proposed an
equation of motion
that
is motivated by the physics and seems to capture a number of the essential
features
of the observations.  The equation is written in cylindrical geometry and is for
$R(\theta,t)$ which is the modulus of the radius vector on the flame front:
\begin{eqnarray}
{\partial R \over \partial t}&=&
 {U_b\over 2{R_0}^2(t)}\left({\partial R \over \partial \theta }\right)^2
 +{D_M\over {R_0}^2(t)}{\partial^2 R\over \partial\theta^2}\\ \nonumber &+&
{\gamma
 U_b\over 2R_0 (t)} I(R)+U_b \ . \label{Eqdim1e}
\end{eqnarray}
Here 0$ <\theta <  2\pi$ is an angle and the constants $U_b,D_M$ and
$\gamma$ are the
front velocity for an ideal cylindrical front, the Markstein diffusivity
and the thermal
expansion coefficient respectively. $R_0(t)$ is the mean
radius of the propagating flame:
\begin{equation}
R_0 (t)={1\over 2\pi}\int_{0}^{2\pi}R(\theta,t)d\theta \  .
\label{R0e}
\end{equation}
The functional $I(R)$ is best represented in terms
of its Fourier decomposition. Its Fourier component is $|k|R_k$ where $R_k$
is the
Fourier component of $R$.

Numerical simulations of the type reported in ref.\cite{94FSF} are presented in
Fig.4.1.
The two
most prominent features of these simulations are the wrinkled multi-cusp
appearance
of the fronts and its acceleration as time progresses. One observes the
phenomenon
of tip splitting in which new cusps are added to the
growing fronts between existing cusps. Both experiments and simulations
indicate that for large times $R_0$ grows as a power in time
\begin{equation}
R_0(t) = (const+t)^{\beta} \ , \label{accele}
\end{equation}
with $\beta>1$, (of the order of $1.5$) and that the width of the interface $W$
grows with $R_0$ as
\begin{equation}
W(t) \sim R_0(t)^\chi \ , \label{scalinge}
\end{equation}
with $\chi<1$ (of the order of 2/3). The understanding of these two
features and
the derivation of the
scaling relation between $\beta$ and $\chi$ are the main aims of this chapter.

Equation (\ref{Eqdim1e}) can be written as a one-parameter
equation by rescaling $R$ and $t$ according to $r\equiv RU_b/
D_M$,  $\tau\equiv tU_b^2/ D_M$. Computing the derivative of
Eq.(\ref{Eqdim1e}) with respect to $\theta$ and substituting the
dimensionless variables one obtains:
\begin{equation}
{\partial u \over \partial \tau}={u \over r_{0}^2}
   {\partial u \over \partial \theta}+{1\over r_{0}^2}{\partial^2u
   \over \partial \theta^2}+{\gamma\over 2 r_0}I\{ u\} \ . \label{eqfinal1e}
\end{equation}
where $u\equiv {\partial r \over \partial \theta}$. To complete
this equation we need a second one for $r_0(t)$, which is obtained
by averaging (\ref{Eqdim1e}) over the angles and rescaling as
above. The result is
\begin{equation}
{dr_0 \over d\tau}={1  \over 2r_{0}^2}{1 \over
2\pi}\int_{0}^{2\pi}u^2d\theta +1 \ . \label{eqr01e}
\end{equation}
These two equations are the basis for further analysis

Following \cite{82LC,85TFH,90J,84BF,89J,95J} we expand now the solutions
$u(\theta,\tau)$
in
poles whose position $z_j(\tau)\equiv x_j(\tau)+iy_j(\tau)$ in the complex
plane
is time dependent:
\begin{eqnarray}
u(\theta,\tau)&=&\sum_{j=1}^{N}\cot \left[{\theta-z_j(\tau) \over 2}\right]
   + c.c.  \label{upoles1e} \\
&=&\sum_{j=1}^{N}{2\sin [\theta-x_j(\tau)]\over
\cosh [y_j(\tau)]-\cos [\theta-x_j(\tau)]}\ , \nonumber
\end{eqnarray}
\begin{equation}
r(\theta,\tau)=2\sum_{j=1}^{N}{\ln \Big[\cosh (y_j(\tau))-\cos
(\theta-x_j(\tau)) \Big]}+C(\tau) \ . \label{rpoles1e}
\end{equation}
In (\ref{rpoles1e}) $C(\tau)$ is a function of time. The function
(\ref{rpoles1e}) is a superposition of quasi-cusps (i.e. cusps
that are rounded at the tip). The real part of the pole position
(i.e. $x_j$) describes the angle coordinate of the maximum of the
quasi-cusp, and the imaginary part of the pole position (i.e
$y_j$) is related the height of the quasi-cusp. As $y_j$ decreases
(increases) the height of the cusp increases (decreases). The
physical motivation for this representation of the solutions
should be evident from Fig.4.1.

The main advantage of this representation is that the propagation
and wrinkling of the front can be described now via the dynamics
of the poles and of $r_0(t)$. Substituting (\ref{upoles1e}) in
(\ref{eqfinal1e}) we derive the following ordinary differential
equations for the positions of the poles:
\begin{equation}
- r_0^2{dz_{j}\over d\tau}=\sum_{k=1
  ,k\neq j}^{2N }\cot \left({z_j-z_k\over 2}\right)
  +i{\gamma r_0 \over 2 }sign [Im(z_j)] \ . \label{eqsze}
\end{equation}

After substitution of (\ref{upoles1e}) in (\ref{eqr01e}) we get,
using (\ref{eqsze}) the ordinary differential equation for $r_0$,
\begin{equation}
{dr_0\over d\tau}=2\sum_{k=1}^N {dy_k\over d\tau}+2\left( {\gamma\over 2}{N\over
     r_0}-{N^2\over r_0^2}\right) +1 \ . \label{r1polee}
 \end{equation}


In our problem the outward growth introduces important modifications to the
channel results.
The number of poles in a stable configuration is proportional here to the
radius $r_0$
instead of $L$, but the former
grows in time. The system becomes therefore unstable to the addition of new
poles. If there
is noise in the system that can generate new poles, they will not be pushed
toward infinite
$y$. It is important to stress that any infinitesimal noise (either
numerical or experimental)
is sufficient to generate new poles. These new poles do not necessarily
merge their
$x$-positions with existing cusps.
Even though there is attraction along the real axis as in the channel case,
there is a
stretching of the distance between the poles due to the
radial growth. This may counterbalance the attraction. Our first new idea
is that these two opposing
tendencies define a typical scale denoted as $\cal L$. if we have a cusp
that is made
from the $x$-merging of $N_c$ poles on the line $x=x_c$ and we want to know
whether a
$x$-nearby pole with real coordinate $x_1$ will
merge with this large cusp, the answer depends on the distance $D=r_0|x_c-x_1|$.
There is a length ${\cal L}(N_c,r_0)$ such that if $D>{\cal L}(N_c,r_0)$
then the
single cusp will never merge with the larger cusp. In the opposite limit
the single
cusp will move towards the large cusp until their $x$- position merges and the
large cusp will have $N_c+1$ poles.

This finding stems directly from the equations of motion of the
$N_c$ $x$-merged poles and the single pole at $x_1$. First note
that from Eq.\ref{accele} (which is not explained yet) it follows
that asymptotically $r_0(\tau)=(a+\tau)^\beta$ where
$r_0(0)=a^\beta$. Next start from \ref{eqsze} and write equations
for the angular distance $x=x_1-x_c$. It follows that for any
configuration $y_j$ along the imaginary axis
\begin{equation}
{dx\over d\tau}\le -{2N_c\sin {x} [ 1-\cos{x}]^{-1} \over
   (a+\tau)^{2\beta}}=-{2N_c\cot({x\over 2}) \over (a+\tau)^{2\beta}}\ .
\label{N+1e}
 \end{equation}
For small x we get
\begin{equation}
{dx\over d\tau}\le -{4N_c\over x(a+\tau)^{2\beta}}\ .\label{Dpte}
\end{equation}
The solution of this equation is
\begin{equation}
x(0)^2-x(\tau)^2\ge {8N_c \over 2 \beta
-1}(a^{1-2\beta}-(a+\tau)^{1-2\beta})\ . \label{xtaue}
\end{equation}
To find ${\cal L}$ we set $x(\infty) > 0$ from which we find that
the angular distance will remain finite as long as
\begin{equation}
x(0)^2 > {8N_c \over 2 \beta -1}a^{1-2\beta}\ . \label{x0e}
\end{equation}
Since $r_0 \sim a^\beta$ we find the threshold angle $x^*$
\begin{equation}
x^* \sim \sqrt N_c r_0^{{(1 - 2\beta) \over 2\beta}} \ ,
\label{x*2e}
\end{equation}
above which there is no merging between the giant cusp and the isolated pole.
To find the actual distance ${\cal L}(N_c,r_0)$ we multiply the angular
distance
by $r_0$ and find
\begin{equation}
{\cal L}(N_c,r_0) \equiv r_0 x^*  \sim \sqrt{N_c} r_0^{{1\over
2\beta}} \ . \label{ratte}
\end{equation}

To understand the geometric meaning of this result we recall the
features of the TFH cusp solution. Having a typical length $L$ the
number of poles in the cusp is linear in $L$. Similarly, if we
have in this problem two cusps a distance $2 \cal L$ apart, the
number $N_c$ in each of them will be of the order of $\cal L$.
From (\ref{ratte}) it follows that
\begin{equation}
{\cal L} \sim  r_0^{{1\over \beta}} \ . \label{scaling1e}
\end{equation}
For $\beta>1$ the circumference grows faster than $\cal L$, and therefore
at some
points in time poles that appear between two large cusps would not be
attracted toward
either, and new cusps will appear. We will show later that the most
unstable positions  to
the appearance of new cusps are precisely the midpoints between existing
cusps. This is
the mechanism for the addition of cusps in analogy with tip splitting in
Laplacian growth.

We can now estimate the width of the flame front as the height of
the largest cusps. Since this height is proportional to $\cal L$
(cf. property (v) of the TFH solution), Eq.(\ref{scaling1e}) and
Eq.(\ref{scalinge}) lead to the scaling relation
\begin{equation}
\chi = 1/\beta \ . \label{scalrele}
\end{equation}
This scaling law is expected to hold all the way to $\beta=1$ for which the
flame front
does not accelerate and the size of the cusps becomes proportional to $r_0$.









In channels there is a natural lengthscale, the width $\tilde L$ of the
channel. The
translation of channel results to radial geometry will be based on the
identification
in the latter context of the time dependent scale ${\cal L}(t)$ that plays
the role of
$\tilde L$ in the former. To do this we need first to review briefly the
main pertinent results
for noisy channel growth. In channel geometry the equation of motion is
written in terms
of the position $h(x,t)$ of the
flame front above the $x$-axis. After appropriate rescalings \cite{85TFH} it
reads:
\begin{equation}
{\partial h(x,t) \over \partial t}=\!
{1\over 2}\!\left[{\partial h(x,t) \over \partial x }\right]^2
 \!\!+\!\!\nu{\partial^2 h(x,t)\over \partial x^2}+ I\{h(x,t)\}\!+\!1.
\label{Eqnondire}
\end{equation}
It is convenient to rescale the domain size further to $0<\theta<2\pi$, and
to change
variables to $u(\theta,t)\equiv {\partial h(\theta,t)/\partial\theta}$.
In terms of this function we find
\begin{equation}
{\partial u(\theta,t) \over \partial t}\!=\! {u(\theta,t)\over
L^2}{\partial u(\theta,t) \over \partial \theta } \!+\!\!{\nu\over
L^2}{\partial^2 u(\theta,t)\over \partial \theta^2}\!+ \!\!{1\over
L}I\{u(\theta,t)\} \label{eque}
\end{equation}
where $L=\tilde L/2\pi$. In noiseless conditions this equation admits exact
solutions
that are represented in terms of $N$ poles whose position $z_j(t)\equiv
x_j(t)+iy_j(t)$
in the complex plane is time dependent:
\begin{equation}
u(\theta,t)=\nu\sum_{j=1}^{N}\cot \left[{\theta-z_j(t) \over 2}\right]
   + c.c.\ , \label{bpolese}
\end{equation}
The steady state for channel propagation is unique and linearly
stable; it consists of $N(L)$ poles which are aligned on one line
parallel to the imaginary axis. The geometric appearance of the
flame front is a giant cusp, analogous to the single finger in the
case of Laplacian growth in a channel. The height of the cusp is
proportional to $L$, and the propagation velocity is a constant of
the motion. The number of poles in the giant cusp is linear in $L$
Eq. (\ref{NofLe},

The introduction of additive random noise to the dynamics changes the
picture qualitatively. It is convenient to add noise to the equation of
motion in Fourier
representation by adding
a white noise $\eta_k$ for every $k$ mode. The noise correlation function
satisfies the relation
$<\eta_k(t)\eta_{k'}(t')>=\delta_{k,k'}\delta(t-t')f/L$. The noise in our
simulations is taken from a flat distribution
in the interval $[-\sqrt{2f/L},\sqrt{2f/L}]$;  this guarantees
that when the system size changes, the typical noise per unit
length of the flame front remains constant. It was shown in chapter 2
and \cite{OGKP} that for moderate
but fixed noise levels
the average velocity $v$ of the front increases with $L$ as a power law.
In our present simulations we found
\begin{equation}
v\sim L^{\mu} \ , \quad \mu\approx 0.35\pm 0.03 \ .
\label{vlScalee}
\end{equation}
For a fixed system size $L$ the velocity has also a power law dependence on the
level of the noise, but with a much smaller exponent:
$v\sim f^\xi \ , \quad \xi\approx 0.02$.
These results were understood theoretically by analysing the noisy creation of
new poles that interact with the poles defining the giant cusp (in
chapter 2 and \cite{OGKP}).












Next we shed light on phenomenon of tip splitting that here is seen as the
addition
of new cusps roughly in between existing ones.  We mentioned the
instability toward the
addition of
new poles. We argue now that the tip between the cusps is most sensitive to
pole creation.
This can be shown in both channel and radial geometry. For example
consider a TFH-giant cusp
solution in which all the poles are aligned (without loss of generality) on
the $x=0$
line. Add a new pole in the complex position $(x_a,y_a)$
to the existing $N(L)$ poles, and study its
fate. It can be shown that in the limit $y_a \to \infty$ (which is the
limit of a
vanishing perturbation of the solution)
the equation of motion is
\begin{equation}
{dy_a \over dt} = {2\pi\nu \over L^2}(2N(L)+1)-1   \quad\quad y_a
\to \infty \ .  \label{yinf1e}
\end{equation}
Since $N(L)$ satisfies (\ref{NofLe}) this equation can be
rewritten as
\begin{equation}
{dy_a \over dt} = {4\pi\nu \over L^2}(1-\alpha)    \quad\quad y_a \to \infty\ ,
 \label{yinf2e}
\end{equation}
where $\alpha=( L/(2\pi\nu)+1)/2 -N(L)$. Obviously $\alpha \le 1$ and it is
precisely
$1$ only when $L$ is $L=(2n+1)2\pi \nu$.  Next it can be shown that
for $y_a$ much larger than $y_{N(L)}$ but not infinite the following is true:
\begin{eqnarray}
{dy_a \over dt} &>& \lim_{y_a\to \infty} {dy_a \over dt} \quad x_a=0 \\
 {dy_a \over dt} &<& \lim_{y_a\to \infty} {dy_a \over dt} \quad x_a=\pi
 \end{eqnarray}
 We learn from these results that there exist values of $L$ for which a pole
 that is
 added at infinity will have marginal attraction ($dy_a/dt=0$).
 Similar understanding can be obtained from a standard stability analysis
 without using
 pole decomposition. Perturbing a TFH-cusp solution we find linear equations
 whose
 eigenvalues $\lambda_i$ can be obtained by standard numerical techniques:
 (i) all $Re(\lambda_i)$ are non-positive.
 (ii) at the isolated values of $L$ for which $L=(2n+1)2\pi\nu$
 $Re(\lambda_1)$ and
 $Re(\lambda_2)$ become
 zero (note that due to the logarithmic scale the zero is not evident)
 (iii) There exists a general tendency of all $Re(\lambda_i)$ to approach
 zero in absolute magnitude such as ${1 \over L^2}$ from
 below as $L$ increases. This indicates a growing sensitivity to noise when
 the system
 size increases. (iv) There exists a Goldsone mode $\lambda_0=0$ due to
 translational
 invariance.

 The upshot of this discussion is that finite perturbations
 (i.e. poles at finite $y_a$) will grow if the $x$ position of the pole is
 sufficiently
 near the tip. The position $x=\pi$ (the tip of the finger) is the most
 unstable one.
 In the channel geometry this means that noise results in the appearance
 of new cusps at the tip of the fingers, but due to the attraction to the
 giant cusp      they
 move toward $x=0$ and disappear in the giant cusp. In fact, one sees in
 numerical
 simulations a train of small
 cusps   that move toward the giant cusp. Analysis shows that at the same time
 the furthest
 pole at $y_{N(L)}$ is pushed towards infinity. Also in cylindrical geometry
 the most sensitive position to the appearance of new cusps is right between
 two existing
 cusps independently if the system is marginal (the total number of poles
 fits the radius)
 or unstable (total number of poles is too small at a given radius). Whether
 or not the
 addition of a new pole results in tip splitting depends on their $x$ position.
 When the distance from existing cusps is larger
 than ${\cal L}$ the new poles that are generated by noise will
 remain near the tip between the two cusps and will cause tip splitting.



















The picture used remains valid
as long as the poles that are introduced by the noisy perturbation do not
destroy the identity
of the giant cusp. Indeed, the numerical simulations show that in the
presence of moderate
noise the additional poles appear as smaller cusps that are constantly
running towards
the giant cusp. Our point here, is not to predict the numerical values of the
scaling exponents in the {\em channel} (this was done in ref.\cite{OGKP}
and chapter 2,
but to use them to predict the scaling exponents characterizing the
acceleration and the
geometry of the flame front in {\em radial} geometry.

Superficially it seems that in radial geometry the growth pattern is
qualitatively different.
In fact, close observation of the growth patterns (see Fig.4.1) shows that
most of the time
there exist some big cusps that attract other smaller cusps,
but that every
now and then ``new" big cusps form and begin to act as local absorbers of
small cusps
that appear randomly.  The understanding of this phenomenon gives the clue
how to
translate results from channels to radial growth.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure}
 \epsfxsize=6.5truecm
 \epsfbox{zeevchan1.ps}
 \caption{Simulations of the outward propagating flame front. Note that
there is a wide distribution of cusp sizes.} \label{fig:fig1e}
 \end{figure}

%%%%%%%%%%%%%%%%%%%%
 Equations (\ref{eqfinal1e}), (\ref{eqr01e})  again admit exact solutions in terms of poles, of the form
of Eq.(\ref{eqsze}). It is easy write down the equations of motion
of the poles and check that the poles are attractive along the
real direction (which means physically that they are attracted
along the angular coordinate) but they are repulsive along the
imaginary direction, which is associated with the radial
coordinate. If it were not for the stretching that is caused by
the increase of the radius (and with it the perimeter), all the
poles would have coalesced into one giant cusp. Thus we have a
competition between pole attraction and stretching. Since the
attraction decreases with the distance between the poles in the
angular directions, there is always an initial  critical length
scale above which poles cannot coalesce their real coordinates
when time progresses.

Suppose now that noise adds new poles to the system. The poles do
not necessarily
merge their real positions with existing cusps. If we have a large cusp
made from the merging
of the real coordinates $x_c$ of $N_c$ poles, we want to know whether a
nearby pole with real
coordinate $x_1$ will merge with this large cusp. The answer will depend of
course on the
distance $D\equiv r_0|x_c-x_1|$. A direct calculation \cite{KOP95}, using
the equation
of motions for the
poles shows that there exists a critical length ${\cal L}(r_0)$ such
that if $D>{\cal L}(r_0)$
the single pole never merges with the giant cusp. The result of the
calculation is that
\begin{equation}
{\cal L}\sim r_0^{1/\beta} \ . \label{Lbeta2e}
\end{equation}
Note that a failure of a single pole to be attracted to a large cusp
means that tip-splitting has occurred. This is the exact analog of tip-splitting
in Laplacian growth.

It is now time to relate the channel and radial geometries. We
identify the typical scale in the radial geometry as ${\cal L}\sim
W\sim r_0^\chi$. On the one hand this leads to the scaling
relation $\beta=1/\chi$. On the other hand we use the result
established in a channel, (\ref{vlScalee}), with this
identification of a scale, and find $\dot  r_0 = r_0 ^{\chi \mu}$.
Comparing with (\ref{accele}) we find:
\begin{equation}
\beta = {1\over (1- \chi \mu)} \ . \label{betamue}
\end{equation}

This result leads us to expect two dynamical regimes for our
problem. Starting from smooth initial conditions, in relatively
short times the roughness exponent remains close to unity. This is
mainly since the typical scale ${\cal L}$ is not relevant yet, and
most of the poles that are generated by noise merge into a few
larger cusps. In later times the roughening exponent settles at
its asymptotic value, and all the asymptotic scaling relations
used above become valid. We thus expect $\beta$ to decrease from
$1/(1-\mu)$ to an asymptotic value determined by $\chi=1/\beta$ in
(\ref{betamue}):
\begin{equation}
\beta=1+\mu \approx 1.35 \pm 0.03 \ . \label{predbetae}
\end{equation}
The expected value of $\chi$ is thus $\chi=0.74\pm 0.03$.
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
 \epsfxsize=6.5truecm
\epsfbox{zeevchan2.ps}
% \vspace{.5cm}
\caption{Panel a: a logarithmic plot of the velocity versus time for a
radially evolving
 system. The parameters
of the simulation are: $f=10^{-8}$, $\gamma=0.8$, $\nu=1$. Panel
b:Logarithmic plot of the width of the flame front as a function
of the mean radius.} \label{fig:fig2e}
\end{figure}
%%%%%%%%%%%%%%%%%%%%
We tested these predictions in numerical simulations. We
integrated Eq.(\ref{eque}), and in Fig.4.2 we display the results
for the growth velocity as a function of time.  After a limited
domain of exponential growth we observe a continuous reduction of
the time dependent exponent. In the initial region we get $\beta
= 1.65\pm 0.1$ while in the final decade of the temporal range we
find $\beta  = 1.35 \pm 0.1$. We consider this a good agreement
with
 (\ref{predbetae}).
 A second important test is provided by measuring the width of the system as
a function of the radius, see Fig.4.2b. Again we observe a cross-over related to
the initial dynamics; In the last temporal decade the exponent settles at
$\chi= 0.75\pm .1$.
We conclude that at times large enough to observe the asymptotics our
 predictions
are verified.

Finally, we stress some differences between radial and channel geometries.
Fronts in a channel exhibit mainly one giant cusp which is only marginally
disturbed by the small cusps that are introduced by noise. In the radial
geometry, as can be concluded from the discussion above, there exist at
any time cusps of all sizes from the smallest to the largest. This broad
distribution of cusps (and scales) must influence correlation function
in ways that differ qualitatively from correlation functions computed in
channel geometries.
%%%%%%%%%%%%%%%%%%%%
\begin{figure}
 \epsfxsize=6.5truecm
\epsfbox{zeevchan3.ps}
\caption{Panel a: a logarithmic plot of the correlation function F(y) of the
interface versus the distance y between points.
Panel b: Second derivative of the correlation function -F''(l)
of the interface versus the distance l between points.}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%
To make the point clear we exhibit in Fig.4.3a the structure function
\begin{equation}
F(y)\equiv \sqrt{\left< |R(x+y)-R(x)|^2\right >} \label{Fe}
\end{equation}
computed for a typical radial front, with $x=R\theta$. To stress the
scaling region we exhibit
the second derivative of this function in Fig.4.3b. The low end of the
graph can be fitted well by a power law $y^{-\alpha}$ with $\alpha\approx 0.6$.
This indicates that $F(y)\approx Ay +By^{2-\alpha}$. In a channel
geometry we get entirely different structure functions that do not exhibit such
scaling functions at all. The way to understand this behavior in the radial
geometry is to consider a distribution of cusps that remain distinct from
each other but whose scales are distributed according to some distribution
$P^{\prime}(\ell)$. Let us define a distribution function
$P(\ell) \sim \ell P^{\prime}(\ell)$ which give us the probability that a
point on the circuit with the mean radius lies on the basis of the cusp with the
size $\ell$.
For each of these cusps there is a contribution to the correlation function
of the form $f(y,\ell)\approx \ell g(y/\ell)$ where $g(x)$ is a scaling
function,
$g(x)\approx x$ for $x<1$ and $g(x)\approx$ constant for $x>1$. The total
correlation
can be estimated (when the poles are distinct) as
\begin{equation}
F(y)\approx \sum_\ell P(\ell)\ell g(y/\ell) \ .
\end{equation}
The first derivative leaves us with $\sum_\ell P(\ell)g'(y/\ell)$, and using
the fact that $g'$ vanishes for $x>1$ we estimate $F'(y)=\sum_{\ell=y}^W
P(\ell)$.
The second derivative yields $F''(y)\approx - P(y)$. Thus the structure
function is
determined by the scale distribution of cusps, and if the latter is a power law,
this should be seen in the second derivative of $F(y)$ as demonstrated in
Fig.4.3.
The conclusion of this analysis is that the radial case exhibits a scaling
function that characterizes the distributions of cusps, $P(\ell)\approx
\ell^{-\alpha}$.

\section{Conclusions}
The main purpose of this chapter was to find exponents of the
problem and find connections between them. Using the main result
of  the channel case (dependence of the velocity on the channel
size) we can find the acceleration of the flame front in the
radial case $(R_0(t) = (const+t)^{\beta})$
\begin{equation}
 \beta= 1+\mu \ . \label{iqz1e}
 \end{equation}

 where $\mu$ is the exponent for the dependence of the velocity on the
 channel size
 found before, $\beta$ is the
 acceleration exponent
 and $R_0$ is a mean radius of the flame front.

 Dependence of the width of the flame front in the radial case
 $W(t)$ on mean radius $(R_0(t) = (const+t)^{\beta})$ is
 \begin{equation}
 W(t) \sim R_0(t)^\chi \ . \label{iqz11e}
 \end{equation}

 \begin{equation}
 \chi=1/\beta \ . \label{iqz2e}
 \end{equation}




In summary, we demonstrated that it is possible to use information about
noisy channel dynamics
to predict nontrivial features of the radial evolution, such as the
acceleration and roughening exponents. It would be worthwhile to examine
similar ideas in the context of Laplacian growth patterns.

%\end{document}


==> oleg4.tex <==


\chapter{Laplacian Growth}
\section{Introduction}
The problem of pattern formation is one of the most rapidly developing branches
of nonlinear science today \cite{Pel}. Of special interest is the study of the front dynamics between two phases (interface) that arises in a variety of nonequilibrium physical systems. If, as it usually happens, the motion of the interface is
slow in comparison with the processes that take place in the bulk of both phases
(such as heat transfer, diffusion, etc.), the scalar field governing the evolution of the interface is a harmonic function. It is natural then, to call the
whole process $Laplacian$ $growth$. Depending on the system, this harmonic
scalar field is a temperature (in the freezing of a liquid or Stefan problem),
a concentration (in solidification from a supersaturated solution), an
electrostatic potential (in electrodeposition), a pressure (in flows through porous media), a probability (in diffusion-limited aggregation), etc.

The mathematical problem of Laplacian growth without surface tension exhibits
a family of exact (analytic) solutions in terms of logarithmic poles in the
complex plane. We show that this family of solutions has a remarkable property:
generic initial conditions in channel geometry which begin with arbitrarily
many features exhibit an inverse cascade into a single finger.

In the absence of surface tension, whose effect is to stabilize the
short-wavelength perturbations of the interface, the problem of 2D
Laplacian growth is described as follows

\begin{equation}
(\partial^2_x+\partial^2_y)u=0 \ . \label{oqz2e}
\end{equation}

\begin{equation}
u \mid_{\Gamma(t)}=0 \ , \partial_nu \mid_{\Sigma}=1 \ .
\label{oqz3e}
\end{equation}

\begin{equation}
v_n= \partial_nu \mid_{\Gamma(t)}  \ . \label{oqz4e}
\end{equation}

Here $u(x,y ;t)$ is the scalar field mentioned, $\Gamma(t)$ is the
moving interface, $\Sigma$ is a fixed external boundary, $\partial_n$ is a
component of the gradient normal to the boundary
(i.e. the normal derivative), and $v_n$ is a normal component of the velocity of the front.

We consider an infinitely long interface, obtained by a periodic
continuation of the interface in the channel with periodic
boundary conditions.Then We introduce a time-dependent conformal
map $f$ from the lower half of a ``mathematical" plane, $\xi
\equiv \zeta +i\eta$, to the domain of the physical plane, $z
\equiv x+iy$, where the Laplace equation \ref{oqz2e} is defined as
$\xi \stackrel{f} { \longrightarrow} z$. We also require that
$f(t, \xi ) \approx \xi$ for $ \xi \longrightarrow \zeta-i\infty$.
Thus the function $z=f(t,\zeta)$ describes the moving interface.
From Eqs. (\ref{oqz2e}), (\ref{oqz3e}), (\ref{oqz4e}) for function
$f(t,\xi)$ we obtain the $Laplacian $ $ Growth$ $ Equation$

\begin{equation}
Im ({\partial  f(\xi,t) \over \partial  \xi} { \overline{\partial
f(\xi, t)} \over \partial  t})=1 \mid_{\xi=\zeta-i0} \ , f_{\zeta}
\mid_{\zeta-i\infty}=1 \ . \label{oqz5e}
\end{equation}

Now we will extend these results obtained
for periodic boundary conditions to the
more physical ``no-flux" boundary conditions (no flux across the lateral
boundaries of the channel). This requires that the moving interface orthogonally intersects the walls of the channel. However, unlike the case of periodic boundary conditions, the end points at the two boundaries do not necessarily have the same horizontal coordinate. This is also a periodic problem where the period equals twice the width of the channel. The analysis is the same as before,
but now only half of the strip should be considered as the physical channel,
whereas the second half is the unphysical mirror image.

Let us look for a solution of Eq. (\ref{oqz5e}) in the next form

\begin{eqnarray}
 && f(\xi,t)=\lambda \xi-i{\tau(t)}-
i\sum_{l=1}^N\alpha_l\log(e^{i{\xi}}-e^{i{\xi_l}(t)}),\nonumber\\
&& \sum_{l=1}^N\alpha_l=1- \lambda, -1<\lambda<1 \ , \label{oqz6e}
\end{eqnarray}
where $\tau(t)$ is some real function of time, $\lambda$ is a real constant,
$\alpha_l$ is a complex constant, $\xi_l=\zeta_l+i\eta_l$ denotes the
position of the pole
with the number $l$ and $N$ is the number of poles.

For the  ``no-flux" boundary condition we must add the condition
that for every pole  $\xi_l=\zeta_l+i\eta_l$ with $\alpha_l$ exists a pole
$\xi_l=-\zeta_l+i\eta_l$ with $\overline{\alpha_l}$. So for the function
$F(i{\xi},t)=if(\xi,t)$

\begin{equation}
\overline{F(i{\xi},t)}=F(\overline{i\xi},t)
\end{equation}

We want to prove that the final state will be only one finger.

\section{Asymptotic behavior of the poles in the mathematical plane}

The main purpose of this chapter is to investigate the asymptotic behavior of
the poles in the  mathematical plane.
We want to demonstrate that for time $t\mapsto \infty$, all poles
go to a single point (or two points for no-flux boundary conditions).
The equation for the interface is


\begin{eqnarray}
 && f(\xi,t)=\lambda \xi-i{\tau(t)}-
i\sum_{l=1}^N\alpha_l\log(e^{i\xi}-e^{i{\xi_l}(t)}), \nonumber\\
&& \sum_{l=1}^N\alpha_l=1- \lambda, -1<\lambda<1 \ . \label{oqf1e}
\end{eqnarray}

By substitution of Eq. (\ref{oqf1e}) in the $Laplacian $ $ Growth$
$ Equation$

\begin{equation}
Im ({\partial  f(\xi,t) \over \partial  \xi} { \overline{\partial
f(\xi,t)} \over \partial  t})=1  \mid_{\xi=\zeta-i0} \ ,
\label{oqf2e}
\end{equation}

we can find the equations  of pole motion:

\begin{equation}
const=\tau(t) +(1-\sum^N_{k=1} \overline{\alpha_k})\log {1 \over a_l}
+ \sum^N_{k=1} \overline{\alpha_k} \log({1\over a_l}-\overline{a_k})
  \label{oqf3e}
\end{equation}

and

\begin{equation}
\tau=t-{1 \over 2} \sum^N_{k=1} \sum^N_{l=1} \overline{\alpha_k}
\alpha_l \log(1- \overline{a_k} a_l)+C_0 \ , \label{oqf4e}
\end{equation}
where $a_l=e^{i\xi_l}$.


From eq. (\ref{oqf3e}) we can find

\begin{equation}
 C_1=(1-\lambda) \tau -\sum^N_{l=1}\alpha_l
\log a_l+\sum^N_{k=1} \sum^N_{l=1} \overline{\alpha_k} \alpha_l
\log(1- \overline{a_k} a_l) \ . \label{oqf6e}
\end{equation}
From eqs. (\ref{oqf4e}) and (\ref{oqf6e}) we can obtain

\begin{equation}
 Im(\sum^N_{l=1}\alpha_l\log a_l)=constant  \label{oqf7e}
\end{equation}

and

\begin{equation}
 t=({1+\lambda \over 2})\tau +{1 \over 2}Re(\sum^N_{l=1}\alpha_l\log a_l)
+C_1/2 \ , \label{oqf8e}
\end{equation}
where $\alpha_l$ is a constant, $\xi_l(t)$ is the position of the poles,
$a_l=
e^{i{\xi_l}(t)}$ , and $\lambda+
1 \over 2$
is the portion of the channel occupied by the moving liquid. We will see that
for $\tau \mapsto \infty$ we obtain one finger with wide $\lambda+1 \over 2$.



In Appendix A we will prove from eq.(\ref{oqf4e}) that  $\tau
\mapsto \infty$, if $t \mapsto \infty$ and if  any finite time
singularity does not exist.

The equations of pole motion are next from eq. (\ref{oqf3e})

\begin{equation}
const=\tau+i\overline{\xi_k}
+\sum_l\alpha_l\log(1-e^{i(\xi_l-\overline{\xi_k})}) ,
\label{aqf9e}
\end{equation}

\begin{equation}
 const=\zeta_k+\sum_l(\alpha_l^{\prime\prime}\log
 \mid 1-e^{i(\xi_l-\overline{\xi_k})}\mid+\alpha_l^{\prime}
 \arg(1-e^{i(\xi_l-\overline{\xi_k})})),  \label{oqf9e}
\end{equation}

\begin{equation}
 const={\tau}+\eta_k+\sum_l(\alpha_l^{\prime}\log
  \mid 1-e^{i(\xi_l-\overline{\xi_k})}\mid-\alpha_l^{\prime\prime}
   \arg(1-e^{i(\xi_l-\overline{\xi_k})})),  \label{oqf10e}
\end{equation}

\begin{equation}
   \xi_l=\zeta_l+i\eta_l, \eta_l>0 \ .  \label{oqf11e}
\end{equation}

\begin{equation}
  \alpha_l=\alpha_l^{\prime}+i\alpha_l^{\prime\prime}
\end{equation}

   Let us examine

\begin{equation}
   \arg(1-e^{i(\xi_l-\overline{\xi_k}})=
   \arg([1-e^{i(\zeta_l-\zeta_k)}
   e^{-(\eta_l+\eta_k)}])=\arg[1-a_{lk}e^{i\varphi_{lk}}]  \label{oqf13e}
\end{equation}

\begin{equation}
   \varphi_{lk}=\zeta_l-\zeta_k, a_{lk}=e^{-(\eta_l+\eta_k)}  \label{oqf14e}
\end{equation}


   $\arg[1-a_{lk}e^{i\varphi_{lk}}]$ is a singlevalued
   function of $\varphi_{lk}$, i.e.

\begin{equation}
    -{\pi \over 2}\leq \arg[1-a_{lk}e^{i\varphi_{lk}}]\leq{\pi \over 2}
   \ . \label{oqf15e}
\end{equation}
   From the eq. (\ref{oqf10e} )   the only way to compensate
   for the  divergence of
   term $\tau$ is that
   $\eta_k \mapsto 0$  for $\tau\mapsto \infty,1\leq k \leq N$.


   We want to investigate asymptotic behavior of poles $\tau\mapsto \infty$.
   To eliminate the divergent term $\log \mid 1-e^{i(\xi_k-
   \overline{\xi_k})}\mid$ we multiply eq. (\ref{oqf10e}) by
   $\alpha_k^{\prime\prime}$ and  eq. (\ref{oqf9e}) by $\alpha_k^{\prime}$
   and take difference

\begin{eqnarray}
&& const=\alpha_k^{\prime}\zeta_k-
 \alpha_k^{\prime\prime}\tau+\sum_{l \neq k}
 ((\alpha_l^{\prime\prime}\alpha_k^{\prime}
 -\alpha_k^{\prime\prime}\alpha_l^{\prime})\log
   \mid 1-e^{i(\xi_l-\overline{\xi_k})}\mid+ \nonumber\\ &&
   (\alpha_l^{\prime}\alpha_k^{\prime}+
   \alpha_l^{\prime\prime}\alpha_k^{\prime\prime})
      \arg(1-e^{i(\xi_l-\overline{\xi_k})})).  \label{aqf10e}
      \end{eqnarray}

 We have the divergent terms  $\alpha_k^{\prime\prime}\tau$ in this equation.
 We may assume that for $t \mapsto \infty$,  $N^{\prime}$ groups of poles
      exist to eliminate the divergent terms
           ($\varphi_{lk} \mapsto 0$ for all members of a group).
        $N_l$ is the number of poles in each group, $1< l < N^{\prime}$.
         For each group by
              summation  of eqs. (\ref{aqf10e})
               over all group poles
     we obtain
\begin{eqnarray}
&& const=\alpha_k^{gr\prime}\zeta_k^{gr}-
  \alpha_k^{gr\prime\prime}\tau+\sum_{l \neq k}
   ((\alpha_l^{gr\prime\prime}\alpha_k^{gr\prime}
    -\alpha_k^{gr\prime\prime}\alpha_l^{gr\prime})\log
       \mid 1-e^{i(\xi_l^{gr}-\overline{\xi_k^{gr}})}\mid+\nonumber\\ &&
      (\alpha_l^{gr\prime}\alpha_k^{gr\prime}+
         \alpha_l^{gr\prime\prime}\alpha_k^{gr\prime\prime})
       \arg(1-e^{i(\xi_l^{gr}-\overline{\xi_k^{gr}})})).  \label{aqf11e}
             \end{eqnarray}


\begin{equation}
     \alpha ^{gr\prime\prime}_l=\sum^{N_l}_k\alpha ^{\prime\prime}_k
      \ , \label{oqf50e}
\end{equation}

\begin{equation}
           \alpha ^{gr\prime}_l=\sum^{N_l}_k\alpha ^{\prime}_k
                     \ . \label{oqf51e}
\end{equation}


   We have no merging of these groups  for large $\tau$ and we investigate
   the motion of poles with this assumption

\begin{equation}
   \mid \zeta_l^{gr}-\zeta_k^{gr} \mid \gg \eta_l^{gr} +\eta_k^{gr}  ,
    1\leq l,k\leq N \ . \label{oqf16e}
\end{equation}

For $l\neq k$, $\eta_k^{gr} \mapsto 0$,
  $\varphi_{lk}^{gr}=\zeta_l^{gr}-\zeta_k^{gr}$ we obtain

\begin{equation}
  \log\mid 1-e^{i(\xi_l^{gr}-\overline{\xi_k^{gr}})}\mid\approx
  \log\mid 1-e^{i(\zeta_l^{gr}-\zeta_k^{gr})}\mid=\log2+
  {1\over 2}\log \sin^2 {\varphi_{lk}^{gr}\over 2}   \label{oqf20e}
\end{equation}

and

\begin{equation}
  \arg(1-e^{i(\xi_l^{gr}-\overline{\xi_k^{gr}})})\approx
  \arg(1-e^{i(\zeta_l^{gr}-\zeta_k^{gr})})=
  {\varphi_{lk}^{gr} \over 2}+\pi n-{\pi\over 2} \ . \label{1qf20e}
\end{equation}

  We choose $n$ in Eq.(\ref{1qf20e}) so that Eq.(\ref{oqf15e}) is correct.



  Substituting these  results to the eqs. (\ref{aqf11e})
   we obtain


\begin{eqnarray}
    &&C_k={\alpha^{gr\prime}{\zeta_k^{gr}}}-\alpha^{gr\prime\prime}_k
    \tau+\sum_{l\neq k}[
    ({\alpha^{gr\prime\prime}_l \alpha^{gr\prime}_k}-
    {\alpha^{gr\prime\prime}_k \alpha^{gr\prime}_l})\log \mid \sin
    {\varphi_{lk}^{gr}\over 2}\mid  \nonumber\\ &&
    +(\alpha ^{gr\prime}_l\alpha ^{gr\prime}_k+
    {\alpha ^{gr\prime\prime}_l\alpha ^{gr\prime\prime}_k)}
    {\varphi_{lk}^{gr}\over2}] \label{oqf30e}
\end{eqnarray}



\section{Theorem about coalescence of the poles}

     From eqs. (\ref{oqf30e}) we
     can conclude

    (i) By  summation of eqs.(\ref{oqf30e})
    (or exactly
     from eq.  (\ref{oqf7e}))
     we obtain
\begin{equation}
 \sum_k \alpha_k^{gr\prime} {\zeta_k^{gr}}=const \ . \label{oqf31e}
\end{equation}

    (ii) For $\mid  {\varphi}_{lk}^{gr} \mid
    \mapsto 0,2\pi$, we obtain $\log \mid \sin
     {\varphi_{lk}^{gr}\over 2}\mid \mapsto
     \infty $,
     meaning that the poles can not pass off each other;

     (iii) From (ii) we conclude that $0< \mid \varphi_{lk}^{gr} \mid
     < 2\pi$


     (iv) From (i) and (iii), $\zeta_k^{gr} \mapsto \infty$ is
     impossible;

     (v) In eq.(\ref{oqf30e}) we must compensate the second divergent
     term. From  (iv) and (iii) we can do it only if
     $\alpha ^{gr\prime\prime}_l=\sum^{N_l}_k\alpha ^{\prime\prime}_k=0$
     for all $l$.


    So from eq. (\ref{oqf30e}) we obtain

\begin{equation}
    \sum^{N_l}_k\alpha ^{\prime\prime}_k=0 \ , \label{oqf52e}
\end{equation}

\begin{equation}
     \dot{\varphi^{gr}_{lk}}=0 \ , \label{oqf53e}
\end{equation}

\begin{equation}
     {\varphi^{gr}_{lk}}\neq 0  \ , \label{oqf54e}
\end{equation}

\begin{equation}
     \dot{\zeta^{gr}_k}=0 \ . \label{oqf55e}
\end{equation}

    For the asymptotic  motion of poles in the
    group $N_m$
    we obtain from  eqs. (\ref{oqf52e}),
    (\ref{oqf53e}), (\ref{oqf54e}), (\ref{oqf55e})
    taking leadind terms in eqs. (\ref{oqf8e}), (\ref{aqf9e})

\begin{equation}
\tau={2 \over \lambda+1}t \ , \label{oqf57e}
\end{equation}

\begin{equation}
0=\dot{\tau}+\sum_l^{N_m}\alpha_l { \dot{\eta_k}+ \dot{\eta_l}+i( \dot{\zeta_k}-
 \dot{\zeta_l}) \over
\eta_k+\eta_l+i(\zeta_k-\zeta_l)}
  \ . \label{oqf56e}
\end{equation}




       The solution to these equations  is

\begin{equation}
             \eta_k=\eta_k^0e^{-{1\over \alpha^{gr\prime}_m}{2 \over 1+\lambda
        }t}
        \ , \label{oqf58e}
\end{equation}

\begin{equation}
        \varphi_{lk}={\varphi_{lk}}^0e^{-{1\over \alpha^{gr\prime}_m}
     {2 \over 1+\lambda}t}
     \ , \label{oqf59e}
\end{equation}

\begin{equation}
      \dot{\zeta_k}=0 \ . \label{oqf60e}
\end{equation}

So we may conclude that for eliminating the divergent term we need


\begin{equation}
\alpha ^{gr\prime\prime}_l= \sum^{N_l}_k\alpha
^{\prime\prime}_k=0, \label{orf52e}
\end{equation}

\begin{equation}
\alpha_l^{gr\prime}(1+\lambda)>0
\end{equation}
for all $l$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusions}
With the  periodic boundary condition, eq.(\ref{orf52e}) is
correct for all poles, so we obtain
       $N^{\prime}=1$,
       $m=1$ and $N_m=N$.

       Therefore the unique solution is



\begin{equation}
     \eta_k=\eta_k^0e^{-{2\over (1-\lambda^2)} t} \ , \label{oqf61e}
\end{equation}

\begin{equation}
            \varphi_{lk}={\varphi_{lk}}^0e^{-{2\over (1-\lambda^2)} t}
     \ , \label{oqf62e}
\end{equation}

\begin{equation}
     \dot{\zeta_k}=0 \ . \label{oqf63e}
\end{equation}

\begin{equation}
   1-\lambda^2>0
\end{equation}

With the no-flux boundary condition we have a pair of the poles
whose condition of eq. (\ref{orf52e}) is correct so all these
pairs must merge. Because of the symmetry of the problem these
poles can merge only on the boundaries of the channel $\zeta=0,\pm
\pi$. Therefore we obtain two groups of the poles on boundaries
    $N^{\prime}=2$,
           $m=1,2$, $N_1+N_2=N$, $\alpha^{gr\prime}_1+\alpha^{gr\prime}_2=
           1-\lambda$.

Consequently we obtain the solution (on two boundaries):
\begin{equation}
         \eta_k^{(1)}=\eta_k^{(1),0}e^{-{1\over \alpha^{gr\prime}_1}{2 \over 1+\lambda
             }t}
                     \ , \label{otf58e}
\end{equation}

\begin{equation}
     \varphi_{lk}^{(1)}={\varphi_{lk}}^{(1),0}e^{-{1\over \alpha^{gr\prime}_1}
              {2 \over 1+\lambda}t}
               \ , \label{otf59e}
\end{equation}

\begin{equation}
         {\zeta_k^{(1)}}=0 \ ; \label{otf60e}
\end{equation}

\begin{equation}
\eta_k^{(2)}=\eta_k^{(2),0}e^{-{1\over \alpha^{gr\prime}_2}{2 \over 1+\lambda}t}
       \ , \label{otf581e}
\end{equation}

\begin{equation}
\varphi_{lk}^{(2)}={\varphi_{lk}}^{(2),0}e^{-{1\over \alpha^{gr\prime}_2}
              {2 \over 1+\lambda}t}
                 \ , \label{otf591e}
\end{equation}

\begin{equation}
      {\zeta_k^{(2)}}=\pm \pi \ ; \label{otf601e}
\end{equation}

\begin{equation}
\alpha_1^{gr\prime}(1+\lambda)>0,
\end{equation}

\begin{equation}
\alpha_2^{gr\prime}(1+\lambda)>0.
\end{equation}




\section{Appendix A}
We need to prove that $\tau \mapsto \infty$, if
$t \mapsto \infty$ and if  any finite time singularity does not exist.
This is apparent if the second term in the next formula for $\tau$
 is greater than zero:

\begin{equation}
 \tau=t+[-{1 \over 2} \sum^N_{k=1} \sum^N_{l=1} \overline{\alpha_k} \alpha_l
 \log(1- \overline{a_k} a_l)]+C_0 \ , \label{oqf65e}
\end{equation}
where $\mid a_l \mid <1$ for all $l$.
Let us prove it.

\begin{eqnarray}
 && -{1 \over 2} \sum^N_{k=1} \sum^N_{l=1} \overline{\alpha_k} \alpha_l
\log(1- \overline{a_k} a_l)=-{1 \over 2} \sum^N_{k=1} \sum^N_{l=1}
\overline{\alpha_k} \alpha_l \sum^{\infty}_{n=1}(-{(\overline{a_k} a_l)^n
\over n})
\nonumber\\ && {1 \over 2}\sum^{\infty}_{n=1}{1 \over n}(\sum^N_{k=1}\overline{\alpha_k}
(\overline{a_k})^n)(\sum^N_{l=1}\alpha_l( a_l)^n) \nonumber\\ &&
={1 \over 2}\sum^{\infty}_{n=1}{1 \over n}\overline{(\sum^N_{l=1}\alpha_l( a_l)^n)}(\sum^N_{l=1}\alpha_l( a_l)^n)>0
\end{eqnarray}

